Proving the Turing Universality of Oritatami Co-Transcriptional Folding (Full Text)

We study the oritatami model for molecular co-transcriptional folding. In oritatami systems, the transcript (the "molecule") folds as it is synthesized (transcribed), according to a local energy optimisation process, which is similar to how actual biomolecules such as RNA fold into complex shapes and functions as they are transcribed. We prove that there is an oritatami system embedding universal computation in the folding process itself. Our result relies on the development of a generic toolbox, which is easily reusable for future work to design complex functions in oritatami systems. We develop "low-level" tools that allow to easily spread apart the encoding of different "functions" in the transcript, even if they are required to be applied at the same geometrical location in the folding. We build upon these low-level tools, a programming framework with increasing levels of abstraction, from encoding of instructions into the transcript to logical analysis. This framework is similar to the hardware-to-algorithm levels of abstractions in standard algorithm theory. These various levels of abstractions allow to separate the proof of correctness of the global behavior of our system, from the proof of correctness of its implementation. Thanks to this framework, we were able to computerize the proof of correctness of its implementation and produce certificates, in the form of a relatively small number of proof trees, compact and easily readable and checkable by human, while encapsulating huge case enumerations. We believe this particular type of certificates can be generalized to other discrete dynamical systems, where proofs involve large case enumerations as well.

==> OritatamiTuringPatterns/n=4-L=3-P=1/AppendLineFeedHalt_10__n=4-L=3-P=1.tex <==
%!TEX root = /Users/nschaban/Documents/_Recherche/Pierre-Étienne/oritatami/2018.01.12 ICALP 2018/icalp2018.tex
\newcommand{\AppendLineFeedHaltBlockUZ}[1]{
    \begin{tikzpicture}
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{AppendLineFeedHalt_10__n=4-L=3-P=1-outline.pdf}};
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{AppendLineFeedHalt_10__n=4-L=3-P=1-arrow.pdf}};
        %
        \ifthenelse{\equal{#1}{}}{
\TIKZPointOfInterest{(-1563.75000000*\st pt, 809.73375254*\st pt)}{a}{$(-1,1-h)$}{W}{100.0*\st pt}{Start}{(-1800.00000000*\st pt, -1621.50289790*\st pt)}{8.0}{AppendLineFeedHalt_10__n=4-L=3-P=1-PI-A-_0,0_-begin.pdf}
\TIKZPointOfInterest{(-1363.75000000*\st pt, 1121.50289790*\st pt)}{b}{$\left(3,-\cfrac{3h-5}2\right)$}{E}{100.0*\st pt}{}{(-1200.00000000*\st pt, -1621.50289790*\st pt)}{8.0}{AppendLineFeedHalt_10__n=4-L=3-P=1-PI-B-_4,-72_-top.pdf}
\TIKZPointOfInterest{(1941.25000000*\st pt, 177.53520778*\st pt)}{c}{$(h+c(0),0)$}{E}{100.0*\st pt}{}{(-600.00000000*\st pt, -1621.50289790*\st pt)}{8.0}{AppendLineFeedHalt_10__n=4-L=3-P=1-PI-C-_774,146_-right.pdf}
\TIKZPointOfInterest{(-1546.25000000*\st pt, -458.99346401*\st pt)}{d}{$(h+2,h)$}{E}{100.0*\st pt}{}{(0.00000000*\st pt, -1621.50289790*\st pt)}{8.0}{AppendLineFeedHalt_10__n=4-L=3-P=1-PI-D-_150,293_-mid-right.pdf}
\TIKZPointOfInterest{(-1196.25000000*\st pt, 173.20508076*\st pt)}{e}{$(h-1,1)$}{SE}{75.0*\st pt}{}{(600.00000000*\st pt, -1621.50289790*\st pt)}{8.0}{AppendLineFeedHalt_10__n=4-L=3-P=1-PI-E-_147,147_-left.pdf}
\TIKZPointOfInterest{(-1928.75000000*\st pt, -1095.52213579*\st pt)}{f}{$(h-1,2h)$}{SW}{100.0*\st pt}{}{(1200.00000000*\st pt, -1621.50289790*\st pt)}{8.0}{AppendLineFeedHalt_10__n=4-L=3-P=1-PI-F-_147,440_-bottom.pdf}
\TIKZPointOfInterest{(-1913.75000000*\st pt, -1095.52213579*\st pt)}{g}{$(h+2,2h)$}{NE}{100.0*\st pt}{}{(1800.00000000*\st pt, -1621.50289790*\st pt)}{8.0}{AppendLineFeedHalt_10__n=4-L=3-P=1-PI-G-_150,440_-bottom-right.pdf}
\TIKZPointOfInterest{(-1558.75000000*\st pt, -463.32359102*\st pt)}{h}{$(h,h+1)$}{NW}{100.0*\st pt}{Trapped}{(-1800.00000000*\st pt, -2221.50289790*\st pt)}{8.0}{AppendLineFeedHalt_10__n=4-L=3-P=1-PI-H-_148,294_-b-left.pdf}
\TIKZPointOfInterest{(-1921.25000000*\st pt, -1082.53175473*\st pt)}{i}{$(h-1,2h-3)$}{NW}{100.0*\st pt}{Stop}{(-1200.00000000*\st pt, -2221.50289790*\st pt)}{8.0}{AppendLineFeedHalt_10__n=4-L=3-P=1-PI-I-_147,437_-end.pdf}
            }{}%ifthenelse
%
\node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{AppendLineFeedHalt_10__n=4-L=3-P=1-path.pdf}};
%
            \ifthenelse{\equal{#1}{}}{
\TIKZBLOCKRETURNLINEFEEDHALT{2}{-406.125}{77.726}
            }{}%ifthenelse
%
    \end{tikzpicture}
}%newcommand


==> OritatamiTuringPatterns/n=4-L=3-P=1/Append_10__n=4-L=3-P=1.tex <==
%!TEX root = /Users/nschaban/Documents/_Recherche/Pierre-Étienne/oritatami/2018.01.12 ICALP 2018/icalp2018.tex
\newcommand{\AppendBlockUZ}[1]{
    \begin{tikzpicture}
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{Append_10__n=4-L=3-P=1-outline.pdf}};
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{Append_10__n=4-L=3-P=1-arrow.pdf}};
        %
        \ifthenelse{\equal{#1}{}}{
\TIKZPointOfInterest{(-1967.50000000*\st pt, 478.47903559*\st pt)}{a}{$(-1,1-h)$}{W}{100.0*\st pt}{Start}{(-2100.00000000*\st pt, -1090.24818095*\st pt)}{8.0}{Append_10__n=4-L=3-P=1-PI-A-_0,0_-begin.pdf}
\TIKZPointOfInterest{(-1767.50000000*\st pt, 790.24818095*\st pt)}{b}{$\left(3,-\cfrac{3h-5}2\right)$}{E}{100.0*\st pt}{}{(-1500.00000000*\st pt, -1090.24818095*\st pt)}{8.0}{Append_10__n=4-L=3-P=1-PI-B-_4,-72_-top.pdf}
\TIKZPointOfInterest{(-1590.00000000*\st pt, -140.72912811*\st pt)}{c}{$\left(h-1,-3\right)$}{W}{100.0*\st pt}{}{(-900.00000000*\st pt, -1090.24818095*\st pt)}{8.0}{Append_10__n=4-L=3-P=1-PI-C-_147,143_-write.pdf}
\TIKZPointOfInterest{(-1377.50000000*\st pt, -153.71950917*\st pt)}{d}{$(w+h+1+iW,0)$}{SW}{100.0*\st pt}{Write \word1}{(-300.00000000*\st pt, -1090.24818095*\st pt)}{8.0}{Append_10__n=4-L=3-P=1-PI-D-_191,146_-write1.pdf}
\TIKZPointOfInterest{(-657.50000000*\st pt, -136.39900110*\st pt)}{e}{$((i+1)W+h-7,-4)$}{NW}{50.0*\st pt}{}{(300.00000000*\st pt, -1090.24818095*\st pt)}{8.0}{Append_10__n=4-L=3-P=1-PI-E-_333,142_-write.pdf}
\TIKZPointOfInterest{(-420.00000000*\st pt, -158.04963619*\st pt)}{f}{$(w+h+1+iW,1)$}{SW}{100.0*\st pt}{Write \word0}{(900.00000000*\st pt, -1090.24818095*\st pt)}{8.0}{Append_10__n=4-L=3-P=1-PI-F-_383,147_-write0.pdf}
\TIKZPointOfInterest{(332.50000000*\st pt, -153.71950917*\st pt)}{g}{$(|u|W+h+1,0)$}{SE}{75.0*\st pt}{Start return}{(1500.00000000*\st pt, -1090.24818095*\st pt)}{8.0}{Append_10__n=4-L=3-P=1-PI-G-_533,146_-last.pdf}
\TIKZPointOfInterest{(2017.50000000*\st pt, -153.71950917*\st pt)}{h}{$(|u|W+h+c(|u|),0)$}{E}{100.0*\st pt}{}{(2100.00000000*\st pt, -1090.24818095*\st pt)}{8.0}{Append_10__n=4-L=3-P=1-PI-H-_870,146_-right.pdf}
\TIKZPointOfInterest{(-30.00000000*\st pt, -790.24818095*\st pt)}{i}{$(|u|W+h+2,h)$}{E}{100.0*\st pt}{}{(-2100.00000000*\st pt, -1690.24818095*\st pt)}{8.0}{Append_10__n=4-L=3-P=1-PI-I-_534,293_-bottom-right.pdf}
\TIKZPointOfInterest{(-75.00000000*\st pt, -790.24818095*\st pt)}{j}{$(|u|W+h-7,h)$}{W}{100.0*\st pt}{}{(-1500.00000000*\st pt, -1690.24818095*\st pt)}{8.0}{Append_10__n=4-L=3-P=1-PI-J-_525,293_-bottom-left.pdf}
\TIKZPointOfInterest{(285.00000000*\st pt, -158.04963619*\st pt)}{k}{$(|u|W+h-8,1)$}{SW}{75.0*\st pt}{Next}{(-900.00000000*\st pt, -1690.24818095*\st pt)}{8.0}{Append_10__n=4-L=3-P=1-PI-K-_524,147_-end.pdf}
            }{}%ifthenelse
%
\node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{Append_10__n=4-L=3-P=1-path.pdf}};
%
            \ifthenelse{\equal{#1}{}}{
\TIKZBLOCKAPPENDCARRIAGERETURN{2}{99.500}{223.868}
\TIKZBLOCKAPPENDLETTER{1}{0,0}{-1025.250}{177.535}
\TIKZBLOCKAPPENDLETTER{0}{1,1}{-92.750}{181.865}
            }{}%ifthenelse
%
    \end{tikzpicture}
}%newcommand


==> OritatamiTuringPatterns/n=4-L=3-P=1/Halt_10__n=4-L=3-P=1.tex <==
%!TEX root = /Users/nschaban/Documents/_Recherche/Pierre-Étienne/oritatami/2018.01.12 ICALP 2018/icalp2018.tex
\newcommand{\HaltBlockUZ}[1]{
    \begin{tikzpicture}
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{Halt_10__n=4-L=3-P=1-outline.pdf}};
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{Halt_10__n=4-L=3-P=1-arrow.pdf}};
        %
        \ifthenelse{\equal{#1}{}}{
\TIKZPointOfInterest{(-158.75000000*\st pt, -309.60408185*\st pt)}{a}{$(0,0)$}{NW}{100.0*\st pt}{Start}{(-600.00000000*\st pt, -635.58484397*\st pt)}{8.0}{Halt_10__n=4-L=3-P=1-PI-A-_0,0_-begin.pdf}
\TIKZPointOfInterest{(216.25000000*\st pt, 322.59446291*\st pt)}{b}{$(2,1-h)$}{E}{100.0*\st pt}{}{(0.00000000*\st pt, -635.58484397*\st pt)}{8.0}{Halt_10__n=4-L=3-P=1-PI-B-_2,-146_-top.pdf}
\TIKZPointOfInterest{(201.25000000*\st pt, 322.59446291*\st pt)}{c}{$(-1,1-h)$}{NW}{50.0*\st pt}{Trapped}{(600.00000000*\st pt, -635.58484397*\st pt)}{8.0}{Halt_10__n=4-L=3-P=1-PI-C-_-1,-146_-end.pdf}
            }{}%ifthenelse
%
\node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{Halt_10__n=4-L=3-P=1-path.pdf}};
%
            \ifthenelse{\equal{#1}{}}{
\TIKZBLOCKHALT{2}{121.000}{8.660}
            }{}%ifthenelse
%
    \end{tikzpicture}
}%newcommand


==> OritatamiTuringPatterns/n=4-L=3-P=1/Halt_10_n=4-L=3-P=1-exploded.tex <==
%!TEX root = /Users/nschaban/Documents/_Recherche/Pierre-Étienne/oritatami/2018.01.12 ICALP 2018/icalp2018.tex
\newcommand{\HaltBlockUZnQLTPUexploded}[1]{
\begin{tikzpicture}
%
\ifthenelse{\equal{#1}{}}{
%
\TIKZlabel{(1.25000000*\st pt, 0.00000000*\st pt)}{A\explodedZigZagSize\ZigUp}{NW}{40.0*\st pt}
\TIKZlabel{(141.25000000*\st pt, 311.76914536*\st pt)}{B\explodedZigZagSize\Halt}{SW}{40.0*\st pt}
}{}
%
\node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{Halt_10_n=4-L=3-P=1-exploded.pdf}};
%
\end{tikzpicture}
}%newcommand


==> OritatamiTuringPatterns/n=4-L=3-P=1/Read0_10__n=4-L=3-P=1.tex <==
%!TEX root = /Users/nschaban/Documents/_Recherche/Pierre-Étienne/oritatami/2018.01.12 ICALP 2018/icalp2018.tex
\newcommand{\ReadZBlockUZ}[1]{
    \begin{tikzpicture}
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{Read0_10__n=4-L=3-P=1-outline.pdf}};
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{Read0_10__n=4-L=3-P=1-arrow.pdf}};
        %
        \ifthenelse{\equal{#1}{}}{
\TIKZPointOfInterest{(-472.50000000*\st pt, -303.10889132*\st pt)}{a}{$(0,0)$}{NW}{100.0*\st pt}{Start}{(-1200.00000000*\st pt, -629.08965344*\st pt)}{8.0}{Read0_10__n=4-L=3-P=1-PI-A-_0,0_-begin.pdf}
\TIKZPointOfInterest{(-107.50000000*\st pt, 329.08965344*\st pt)}{b}{$(0,1-h)$}{NW}{50.0*\st pt}{}{(-600.00000000*\st pt, -629.08965344*\st pt)}{8.0}{Read0_10__n=4-L=3-P=1-PI-B-_0,-146_-top-left.pdf}
\TIKZPointOfInterest{(-267.50000000*\st pt, -303.10889132*\st pt)}{c}{$(w-1,0)$}{SE}{50.0*\st pt}{}{(0.00000000*\st pt, -629.08965344*\st pt)}{8.0}{Read0_10__n=4-L=3-P=1-PI-C-_41,0_-w0.pdf}
\TIKZPointOfInterest{(112.50000000*\st pt, 329.08965344*\st pt)}{d}{$(w+2,1-h)$}{NE}{50.0*\st pt}{Read \word0}{(600.00000000*\st pt, -629.08965344*\st pt)}{8.0}{Read0_10__n=4-L=3-P=1-PI-D-_44,-146_-read0.pdf}
\TIKZPointOfInterest{(487.50000000*\st pt, -303.10889132*\st pt)}{e}{$(W,0)$}{NE}{100.0*\st pt}{Next}{(1200.00000000*\st pt, -629.08965344*\st pt)}{8.0}{Read0_10__n=4-L=3-P=1-PI-E-_192,0_-end.pdf}
            }{}%ifthenelse
%
\node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{Read0_10__n=4-L=3-P=1-path.pdf}};
%
            \ifthenelse{\equal{#1}{}}{
\TIKZBLOCKREAD{0}{2}{10}{190.000}{12.990}
            }{}%ifthenelse
%
    \end{tikzpicture}
}%newcommand


==> OritatamiTuringPatterns/n=4-L=3-P=1/Read1_10__n=4-L=3-P=1.tex <==
%!TEX root = /Users/nschaban/Documents/_Recherche/Pierre-Étienne/oritatami/2018.01.12 ICALP 2018/icalp2018.tex
\newcommand{\ReadUBlockUZ}[1]{
    \begin{tikzpicture}
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{Read1_10__n=4-L=3-P=1-outline.pdf}};
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{Read1_10__n=4-L=3-P=1-arrow.pdf}};
        %
        \ifthenelse{\equal{#1}{}}{
\TIKZPointOfInterest{(-641.25000000*\st pt, -322.59446291*\st pt)}{a}{$(0,0)$}{NW}{100.0*\st pt}{Start}{(-1200.00000000*\st pt, -648.57522502*\st pt)}{8.0}{Read1_10__n=4-L=3-P=1-PI-A-_0,0_-begin.pdf}
\TIKZPointOfInterest{(-276.25000000*\st pt, 309.60408185*\st pt)}{b}{$(0,1-h)$}{NW}{50.0*\st pt}{}{(-600.00000000*\st pt, -648.57522502*\st pt)}{8.0}{Read1_10__n=4-L=3-P=1-PI-B-_0,-146_-top-left.pdf}
\TIKZPointOfInterest{(-436.25000000*\st pt, -322.59446291*\st pt)}{c}{$(w-1,0)$}{SE}{50.0*\st pt}{}{(0.00000000*\st pt, -648.57522502*\st pt)}{8.0}{Read1_10__n=4-L=3-P=1-PI-C-_41,0_-w0.pdf}
\TIKZPointOfInterest{(-56.25000000*\st pt, 309.60408185*\st pt)}{d}{$(w+2,1-h)$}{NE}{50.0*\st pt}{Read \word1}{(600.00000000*\st pt, -648.57522502*\st pt)}{8.0}{Read1_10__n=4-L=3-P=1-PI-D-_44,-146_-read1.pdf}
\TIKZPointOfInterest{(678.75000000*\st pt, 309.60408185*\st pt)}{e}{$(W-1,1-h)$}{SE}{100.0*\st pt}{Next}{(1200.00000000*\st pt, -648.57522502*\st pt)}{8.0}{Read1_10__n=4-L=3-P=1-PI-E-_191,-146_-end.pdf}
            }{}%ifthenelse
%
\node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{Read1_10__n=4-L=3-P=1-path.pdf}};
%
            \ifthenelse{\equal{#1}{}}{
\TIKZBLOCKREAD{1}{2}{10}{21.250}{-6.495}
            }{}%ifthenelse
%
    \end{tikzpicture}
}%newcommand


==> OritatamiTuringPatterns/n=4-L=3-P=1/ZagCopy0LineFeed_10__n=4-L=3-P=1.tex <==
%!TEX root = /Users/nschaban/Documents/_Recherche/Pierre-Étienne/oritatami/2018.01.12 ICALP 2018/icalp2018.tex
\newcommand{\ZagCopyZLineFeedBlockUZ}[1]{
    \begin{tikzpicture}
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{ZagCopy0LineFeed_10__n=4-L=3-P=1-outline.pdf}};
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{ZagCopy0LineFeed_10__n=4-L=3-P=1-arrow.pdf}};
        %
        \ifthenelse{\equal{#1}{}}{
\TIKZPointOfInterest{(807.50000000*\st pt, 640.85879880*\st pt)}{a}{$(h-8,1)$}{E}{100.0*\st pt}{start}{(-1500.00000000*\st pt, -953.84917986*\st pt)}{8.0}{ZagCopy0LineFeed_10__n=4-L=3-P=1-PI-A-_0,0_-begin.pdf}
\TIKZPointOfInterest{(442.50000000*\st pt, 8.66025404*\st pt)}{b}{$(h-8,h)$}{E}{150.0*\st pt}{}{(-900.00000000*\st pt, -953.84917986*\st pt)}{8.0}{ZagCopy0LineFeed_10__n=4-L=3-P=1-PI-B-_0,146_-bottom-right.pdf}
\TIKZPointOfInterest{(102.50000000*\st pt, 640.85879880*\st pt)}{c}{$(h-W+w+1,1)$}{NE}{75.0*\st pt}{Read \word0}{(-300.00000000*\st pt, -953.84917986*\st pt)}{8.0}{ZagCopy0LineFeed_10__n=4-L=3-P=1-PI-C-_-141,0_-read0.pdf}
\TIKZPointOfInterest{(-260.00000000*\st pt, 4.33012702*\st pt)}{d}{$(h-W+w+2,1+h)$}{SE}{100.0*\st pt}{Copy \word0}{(300.00000000*\st pt, -953.84917986*\st pt)}{8.0}{ZagCopy0LineFeed_10__n=4-L=3-P=1-PI-D-_-140,147_-copy0.pdf}
\TIKZPointOfInterest{(-122.50000000*\st pt, 640.85879880*\st pt)}{e}{$(h-W-2,1)$}{NE}{175.0*\st pt}{}{(900.00000000*\st pt, -953.84917986*\st pt)}{8.0}{ZagCopy0LineFeed_10__n=4-L=3-P=1-PI-E-_-186,0_-top-left.pdf}
\TIKZPointOfInterest{(-135.00000000*\st pt, 653.84917986*\st pt)}{f}{$(h-W-6,-2)$}{W}{100.0*\st pt}{}{(1500.00000000*\st pt, -953.84917986*\st pt)}{8.0}{ZagCopy0LineFeed_10__n=4-L=3-P=1-PI-F-_-190,-3_-top-left-corner.pdf}
\TIKZPointOfInterest{(-497.50000000*\st pt, 8.66025404*\st pt)}{g}{$(h-W-4,h)$}{NW}{100.0*\st pt}{}{(-1500.00000000*\st pt, -1553.84917986*\st pt)}{8.0}{ZagCopy0LineFeed_10__n=4-L=3-P=1-PI-G-_-188,146_-mid-left.pdf}
\TIKZPointOfInterest{(-845.00000000*\st pt, -627.86841774*\st pt)}{h}{$(h-W,2h)$}{NE}{50.0*\st pt}{Next}{(-900.00000000*\st pt, -1553.84917986*\st pt)}{8.0}{ZagCopy0LineFeed_10__n=4-L=3-P=1-PI-H-_-184,293_-end.pdf}
            }{}%ifthenelse
%
\node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{ZagCopy0LineFeed_10__n=4-L=3-P=1-path.pdf}};
%
            \ifthenelse{\equal{#1}{}}{
\TIKZBLOCKZAGCOPYLINEFEED{0}{2}{10}{145.000}{324.760}
            }{}%ifthenelse
%
    \end{tikzpicture}
}%newcommand


==> OritatamiTuringPatterns/n=4-L=3-P=1/ZagCopy0_10__n=4-L=3-P=1.tex <==
%!TEX root = /Users/nschaban/Documents/_Recherche/Pierre-Étienne/oritatami/2018.01.12 ICALP 2018/icalp2018.tex
\newcommand{\ZagCopyZBlockUZ}[1]{
    \begin{tikzpicture}
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{ZagCopy0_10__n=4-L=3-P=1-outline.pdf}};
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{ZagCopy0_10__n=4-L=3-P=1-arrow.pdf}};
        %
        \ifthenelse{\equal{#1}{}}{
\TIKZPointOfInterest{(632.50000000*\st pt, 298.77876431*\st pt)}{a}{$(h-8,1)$}{E}{100.0*\st pt}{Start}{(-1500.00000000*\st pt, -837.74990748*\st pt)}{8.0}{ZagCopy0_10__n=4-L=3-P=1-PI-A-_0,0_-begin.pdf}
\TIKZPointOfInterest{(267.50000000*\st pt, -333.41978046*\st pt)}{b}{$(h-8,h)$}{E}{150.0*\st pt}{}{(-900.00000000*\st pt, -837.74990748*\st pt)}{8.0}{ZagCopy0_10__n=4-L=3-P=1-PI-B-_0,146_-bottom-right.pdf}
\TIKZPointOfInterest{(-72.50000000*\st pt, 298.77876431*\st pt)}{c}{$(h-W+w+1,1)$}{NE}{100.0*\st pt}{Read \word0}{(-300.00000000*\st pt, -837.74990748*\st pt)}{8.0}{ZagCopy0_10__n=4-L=3-P=1-PI-C-_-141,0_-read0.pdf}
\TIKZPointOfInterest{(-435.00000000*\st pt, -337.74990748*\st pt)}{d}{$(h-W+w+2,1+h)$}{SE}{100.0*\st pt}{Copy \word0}{(300.00000000*\st pt, -837.74990748*\st pt)}{8.0}{ZagCopy0_10__n=4-L=3-P=1-PI-D-_-140,147_-copy0.pdf}
\TIKZPointOfInterest{(-687.50000000*\st pt, -333.41978046*\st pt)}{e}{$(h-W-7,h)$}{NW}{100.0*\st pt}{}{(900.00000000*\st pt, -837.74990748*\st pt)}{8.0}{ZagCopy0_10__n=4-L=3-P=1-PI-E-_-191,146_-bottom-left.pdf}
\TIKZPointOfInterest{(-327.50000000*\st pt, 298.77876431*\st pt)}{f}{$(h-W-8,1)$}{W}{100.0*\st pt}{Next}{(1500.00000000*\st pt, -837.74990748*\st pt)}{8.0}{ZagCopy0_10__n=4-L=3-P=1-PI-F-_-192,0_-end.pdf}
            }{}%ifthenelse
%
\node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{ZagCopy0_10__n=4-L=3-P=1-path.pdf}};
%
            \ifthenelse{\equal{#1}{}}{
\TIKZBLOCKZAGCOPY{0}{2}{10}{-30.000}{-17.321}
            }{}%ifthenelse
%
    \end{tikzpicture}
}%newcommand


==> OritatamiTuringPatterns/n=4-L=3-P=1/ZagCopy1LineFeed_10__n=4-L=3-P=1.tex <==
%!TEX root = /Users/nschaban/Documents/_Recherche/Pierre-Étienne/oritatami/2018.01.12 ICALP 2018/icalp2018.tex
\newcommand{\ZagCopyULineFeedBlockUZ}[1]{
    \begin{tikzpicture}
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{ZagCopy1LineFeed_10__n=4-L=3-P=1-outline.pdf}};
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{ZagCopy1LineFeed_10__n=4-L=3-P=1-arrow.pdf}};
        %
        \ifthenelse{\equal{#1}{}}{
\TIKZPointOfInterest{(807.50000000*\st pt, 640.85879880*\st pt)}{a}{$(h-8,1)$}{E}{100.0*\st pt}{start}{(-1500.00000000*\st pt, -953.84917986*\st pt)}{8.0}{ZagCopy1LineFeed_10__n=4-L=3-P=1-PI-A-_0,0_-begin.pdf}
\TIKZPointOfInterest{(442.50000000*\st pt, 8.66025404*\st pt)}{b}{$(h-8,h)$}{E}{150.0*\st pt}{}{(-900.00000000*\st pt, -953.84917986*\st pt)}{8.0}{ZagCopy1LineFeed_10__n=4-L=3-P=1-PI-B-_0,146_-bottom-right.pdf}
\TIKZPointOfInterest{(102.50000000*\st pt, 640.85879880*\st pt)}{c}{$(h-W+w+1,1)$}{NE}{75.0*\st pt}{Read \word1}{(-300.00000000*\st pt, -953.84917986*\st pt)}{8.0}{ZagCopy1LineFeed_10__n=4-L=3-P=1-PI-C-_-141,0_-read1.pdf}
\TIKZPointOfInterest{(-257.50000000*\st pt, 8.66025404*\st pt)}{d}{$(h-W+w+2,h)$}{SE}{100.0*\st pt}{Copy \word1}{(300.00000000*\st pt, -953.84917986*\st pt)}{8.0}{ZagCopy1LineFeed_10__n=4-L=3-P=1-PI-D-_-140,146_-copy1.pdf}
\TIKZPointOfInterest{(-122.50000000*\st pt, 640.85879880*\st pt)}{e}{$(h-W-2,1)$}{NE}{175.0*\st pt}{}{(900.00000000*\st pt, -953.84917986*\st pt)}{8.0}{ZagCopy1LineFeed_10__n=4-L=3-P=1-PI-E-_-186,0_-top-left.pdf}
\TIKZPointOfInterest{(-135.00000000*\st pt, 653.84917986*\st pt)}{f}{$(h-W-6,-2)$}{W}{100.0*\st pt}{}{(1500.00000000*\st pt, -953.84917986*\st pt)}{8.0}{ZagCopy1LineFeed_10__n=4-L=3-P=1-PI-F-_-190,-3_-top-left-corner.pdf}
\TIKZPointOfInterest{(-497.50000000*\st pt, 8.66025404*\st pt)}{g}{$(h-W-4,h)$}{NW}{100.0*\st pt}{}{(-1500.00000000*\st pt, -1553.84917986*\st pt)}{8.0}{ZagCopy1LineFeed_10__n=4-L=3-P=1-PI-G-_-188,146_-mid-left.pdf}
\TIKZPointOfInterest{(-845.00000000*\st pt, -627.86841774*\st pt)}{h}{$(h-W,2h)$}{NE}{50.0*\st pt}{Next}{(-900.00000000*\st pt, -1553.84917986*\st pt)}{8.0}{ZagCopy1LineFeed_10__n=4-L=3-P=1-PI-H-_-184,293_-end.pdf}
            }{}%ifthenelse
%
\node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{ZagCopy1LineFeed_10__n=4-L=3-P=1-path.pdf}};
%
            \ifthenelse{\equal{#1}{}}{
\TIKZBLOCKZAGCOPYLINEFEED{1}{2}{10}{145.000}{324.760}
            }{}%ifthenelse
%
    \end{tikzpicture}
}%newcommand


==> OritatamiTuringPatterns/n=4-L=3-P=1/ZagCopy1_10__n=4-L=3-P=1.tex <==
%!TEX root = /Users/nschaban/Documents/_Recherche/Pierre-Étienne/oritatami/2018.01.12 ICALP 2018/icalp2018.tex
\newcommand{\ZagCopyUBlockUZ}[1]{
    \begin{tikzpicture}
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{ZagCopy1_10__n=4-L=3-P=1-outline.pdf}};
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{ZagCopy1_10__n=4-L=3-P=1-arrow.pdf}};
        %
        \ifthenelse{\equal{#1}{}}{
\TIKZPointOfInterest{(632.50000000*\st pt, 296.61370080*\st pt)}{a}{$(h-8,1)$}{E}{100.0*\st pt}{Start}{(-1500.00000000*\st pt, -835.58484397*\st pt)}{8.0}{ZagCopy1_10__n=4-L=3-P=1-PI-A-_0,0_-begin.pdf}
\TIKZPointOfInterest{(267.50000000*\st pt, -335.58484397*\st pt)}{b}{$(h-8,h)$}{E}{150.0*\st pt}{}{(-900.00000000*\st pt, -835.58484397*\st pt)}{8.0}{ZagCopy1_10__n=4-L=3-P=1-PI-B-_0,146_-bottom-right.pdf}
\TIKZPointOfInterest{(-72.50000000*\st pt, 296.61370080*\st pt)}{c}{$(h-W+w+1,1)$}{NE}{100.0*\st pt}{Read \word1}{(-300.00000000*\st pt, -835.58484397*\st pt)}{8.0}{ZagCopy1_10__n=4-L=3-P=1-PI-C-_-141,0_-read1.pdf}
\TIKZPointOfInterest{(-432.50000000*\st pt, -335.58484397*\st pt)}{d}{$(h-W+w+2,h)$}{SE}{100.0*\st pt}{Copy \word1}{(300.00000000*\st pt, -835.58484397*\st pt)}{8.0}{ZagCopy1_10__n=4-L=3-P=1-PI-D-_-140,146_-copy1.pdf}
\TIKZPointOfInterest{(-687.50000000*\st pt, -335.58484397*\st pt)}{e}{$(h-W-7,h)$}{NW}{100.0*\st pt}{}{(900.00000000*\st pt, -835.58484397*\st pt)}{8.0}{ZagCopy1_10__n=4-L=3-P=1-PI-E-_-191,146_-bottom-left.pdf}
\TIKZPointOfInterest{(-327.50000000*\st pt, 296.61370080*\st pt)}{f}{$(h-W-8,1)$}{W}{100.0*\st pt}{Next}{(1500.00000000*\st pt, -835.58484397*\st pt)}{8.0}{ZagCopy1_10__n=4-L=3-P=1-PI-F-_-192,0_-end.pdf}
            }{}%ifthenelse
%
\node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{ZagCopy1_10__n=4-L=3-P=1-path.pdf}};
%
            \ifthenelse{\equal{#1}{}}{
\TIKZBLOCKZAGCOPY{1}{2}{10}{-30.000}{-19.486}
            }{}%ifthenelse
%
    \end{tikzpicture}
}%newcommand


==> OritatamiTuringPatterns/n=4-L=3-P=1/ZigCopy0_10__n=4-L=3-P=1.tex <==
%!TEX root = /Users/nschaban/Documents/_Recherche/Pierre-Étienne/oritatami/2018.01.12 ICALP 2018/icalp2018.tex
\newcommand{\ZigCopyZBlockUZ}[1]{
    \begin{tikzpicture}
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{ZigCopy0_10__n=4-L=3-P=1-outline.pdf}};
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{ZigCopy0_10__n=4-L=3-P=1-arrow.pdf}};
        %
        \ifthenelse{\equal{#1}{}}{
\TIKZPointOfInterest{(-632.50000000*\st pt, 298.77876431*\st pt)}{a}{$(-1,1-h)$}{W}{100.0*\st pt}{Start}{(-1500.00000000*\st pt, -837.74990748*\st pt)}{8.0}{ZigCopy0_10__n=4-L=3-P=1-PI-A-_0,0_-begin.pdf}
\TIKZPointOfInterest{(-267.50000000*\st pt, -333.41978046*\st pt)}{b}{$(h-2,0)$}{W}{100.0*\st pt}{}{(-900.00000000*\st pt, -837.74990748*\st pt)}{8.0}{ZigCopy0_10__n=4-L=3-P=1-PI-B-_146,146_-bottom-left.pdf}
\TIKZPointOfInterest{(-407.50000000*\st pt, 298.77876431*\st pt)}{c}{$(w+2,1-h)$}{NW}{100.0*\st pt}{Read \word0}{(-300.00000000*\st pt, -837.74990748*\st pt)}{8.0}{ZigCopy0_10__n=4-L=3-P=1-PI-C-_45,0_-read0.pdf}
\TIKZPointOfInterest{(-45.00000000*\st pt, -337.74990748*\st pt)}{d}{$(h+w+1,1)$}{SE}{100.0*\st pt}{Copy \word0}{(300.00000000*\st pt, -837.74990748*\st pt)}{8.0}{ZigCopy0_10__n=4-L=3-P=1-PI-D-_191,147_-copy0.pdf}
\TIKZPointOfInterest{(-392.50000000*\st pt, 298.77876431*\st pt)}{e}{$(w+5,0)$}{NE}{100.0*\st pt}{\begin{minipage}[t]{2.5cm}\raggedright Start of 2$^{\text{nd}}$ copy unit\end{minipage}}{(900.00000000*\st pt, -837.74990748*\st pt)}{8.0}{ZigCopy0_10__n=4-L=3-P=1-PI-E-_48,0_-2nd-unit.pdf}
\TIKZPointOfInterest{(87.50000000*\st pt, 298.77876431*\st pt)}{f}{$((n-1)(w+6_-1,0)$}{NE}{100.0*\st pt}{\begin{minipage}[t]{2.5cm}\raggedright Start of last copy unit\end{minipage}}{(1500.00000000*\st pt, -837.74990748*\st pt)}{8.0}{ZigCopy0_10__n=4-L=3-P=1-PI-F-_144,0_-last-unit.pdf}
\TIKZPointOfInterest{(687.50000000*\st pt, -333.41978046*\st pt)}{g}{$(W+h-3,0)$}{E}{100.0*\st pt}{}{(-1500.00000000*\st pt, -1437.74990748*\st pt)}{8.0}{ZigCopy0_10__n=4-L=3-P=1-PI-G-_337,146_-bottom-right.pdf}
\TIKZPointOfInterest{(327.50000000*\st pt, 298.77876431*\st pt)}{h}{$(W-1,1-h)$}{E}{100.0*\st pt}{Next}{(-900.00000000*\st pt, -1437.74990748*\st pt)}{8.0}{ZigCopy0_10__n=4-L=3-P=1-PI-H-_192,0_-end.pdf}
            }{}%ifthenelse
%
\node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{ZigCopy0_10__n=4-L=3-P=1-path.pdf}};
%
            \ifthenelse{\equal{#1}{}}{
\TIKZBLOCKZIGCOPY{0}{2}{10}{30.000}{-17.321}
            }{}%ifthenelse
%
    \end{tikzpicture}
}%newcommand


==> OritatamiTuringPatterns/n=4-L=3-P=1/ZigCopy1_10__n=4-L=3-P=1.tex <==
%!TEX root = /Users/nschaban/Documents/_Recherche/Pierre-Étienne/oritatami/2018.01.12 ICALP 2018/icalp2018.tex
\newcommand{\ZigCopyUBlockUZ}[1]{
    \begin{tikzpicture}
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{ZigCopy1_10__n=4-L=3-P=1-outline.pdf}};
        \node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{ZigCopy1_10__n=4-L=3-P=1-arrow.pdf}};
        %
        \ifthenelse{\equal{#1}{}}{
\TIKZPointOfInterest{(-632.50000000*\st pt, 296.61370080*\st pt)}{a}{$(-1,1-h)$}{W}{100.0*\st pt}{Start}{(-1500.00000000*\st pt, -835.58484397*\st pt)}{8.0}{ZigCopy1_10__n=4-L=3-P=1-PI-A-_0,0_-begin.pdf}
\TIKZPointOfInterest{(-267.50000000*\st pt, -335.58484397*\st pt)}{b}{$(h-2,0)$}{W}{100.0*\st pt}{}{(-900.00000000*\st pt, -835.58484397*\st pt)}{8.0}{ZigCopy1_10__n=4-L=3-P=1-PI-B-_146,146_-bottom-left.pdf}
\TIKZPointOfInterest{(-407.50000000*\st pt, 296.61370080*\st pt)}{c}{$(w+2,1-h)$}{NW}{100.0*\st pt}{Read \word1}{(-300.00000000*\st pt, -835.58484397*\st pt)}{8.0}{ZigCopy1_10__n=4-L=3-P=1-PI-C-_45,0_-read1.pdf}
\TIKZPointOfInterest{(-47.50000000*\st pt, -335.58484397*\st pt)}{d}{$(h+w,0)$}{SE}{100.0*\st pt}{Copy \word1}{(300.00000000*\st pt, -835.58484397*\st pt)}{8.0}{ZigCopy1_10__n=4-L=3-P=1-PI-D-_190,146_-copy1.pdf}
\TIKZPointOfInterest{(687.50000000*\st pt, -335.58484397*\st pt)}{e}{$(W+h-3,0)$}{E}{100.0*\st pt}{}{(900.00000000*\st pt, -835.58484397*\st pt)}{8.0}{ZigCopy1_10__n=4-L=3-P=1-PI-E-_337,146_-bottom-right.pdf}
\TIKZPointOfInterest{(327.50000000*\st pt, 296.61370080*\st pt)}{f}{$(W-1,1-h)$}{E}{100.0*\st pt}{Next}{(1500.00000000*\st pt, -835.58484397*\st pt)}{8.0}{ZigCopy1_10__n=4-L=3-P=1-PI-F-_192,0_-end.pdf}
            }{}%ifthenelse
%
\node [anchor=center] () at (0,0) {\includegraphics[scale =\s]{ZigCopy1_10__n=4-L=3-P=1-path.pdf}};
%
            \ifthenelse{\equal{#1}{}}{
\TIKZBLOCKZIGCOPY{1}{2}{10}{30.000}{-19.486}
            }{}%ifthenelse
%
    \end{tikzpicture}
}%newcommand


==> block-coords.tex <==
%!TEX root =  icalp2018.tex

%%%%%----------------
\section{Block coordinates}
%%%%%----------------

Let $\mathcal{S} = (\alpha^0,\alpha^1,\ldots, \alpha^{n-1}; u^0)$ be a skipping cyclic tag system, and for all integer $i \geq 0$, let $t_i$ be the $i^{\text{th}}$ step where $u^{t}$ starts with $\word1$ (starting from $0$, i.e. $t_0$ is the first step where $u^{t_0}$ starts with $\word1$). The following lemma describes the encoding of $\mathcal{S}$ into blocks (i.e. generalises Figure~\ref{fig:example:block:execution} to arbitrary tag systems).

\begin{lemma} \label{lem:actual:ith:row} \label{lem:key}
The (possibly infinite) final block configuration consists of: %(see illustration on Figure~\ref{fig:ith:row})

\newcommand{\theScale}{.7}
\begin{itemize}[nosep]

\item The seed row, i.e. the block \bSEED{$u^0$} ending at coordinates $(-1,0)$.

\item For $i\geq0$, the $i$-th row consists of a zig row located between $y=2(i-1)h+1$ and $y=2ih$, and a zag row located between $y=2ih+1$ and $y=2(i+1)h$, defined as follows:
  \begin{description}[topsep=0pt]
  \item[$\bullet$ \textup{(Compute)} if $u^{1+t_i} = \word0^r1\cdot s$ and if $s\neq\epsilon$ or $\alpha^{1+i+t_{i+1}}\neq\epsilon$:] then ${r = t_{i+1}-t_i-1}$ and:%, as illustrated in Figure~\ref{fig:final:geom:config:compute:1} and~Figure~\ref{fig:final:geom:config:compute:2}:
    \begin{itemize}[itemsep=4pt]
    \item the $i$-th zig-row consists from left to right of the sequence of geometrical blocks whose origin is located at the following coordinates:\\[4pt]
      % \resizebox{\linewidth}{!}{
      \centerline{\hspace*{-1.5cm}\scalebox{\theScale}{
          $\begin{array}{cccccccccc}
             \swarrow y 	&	\multicolumn{4}{c}{2ih} && \multicolumn{4}{c}{(2i-1)h+1}\\ \cmidrule{1-5} \cmidrule{7-10}
             \rightarrow  x	&	ih+(1+t_i)W & \cdots& ih+(t_{i+1}-1)W & ih+t_{i+1}W &  &ih+(1+t_{i+1})W-1  & \cdots & ih+(|s|+t_{i+1})W-1 & ih+(1+|s|+t_{i+1})W-1 \\ \toprule
             \textup{Blocks} & \bnREAD{\word0}{} & \cdots & \bnREAD{\word0}{} & \bnREAD{\word1}{} & & \bnZIGCOPY{$(s_0)$}{} & \cdots & \bnZIGCOPY{$(s_{|s|-1})$}{} & \bnAPPENDRETURN{[\alpha^{1+i+t_{i+1}}]}{}\\
              \midrule
              \textup{Marker}	&	i+1+t_i & \cdots& i+r+t_i & i+t_{i+1} &  & i+1+t_{i+1}  & \cdots & i+1+t_{i+1} & i+1+t_{i+1} 
           \end{array}
           $}}
       \smallskip\\
       This row ends at position $((i+1)h+(1+|s|+|\alpha^{i+1+t_{i+1}}|+t_{i+1})W-7,2ih+2)$.

     \item the $i$-th zag-row consists from left to right of the sequence of geometrical  blocks whose origins are  located at the following coordinates:\\[4pt]
       % \resizebox{\linewidth}{!}{
       \centerline{\hspace*{-1.5cm}\scalebox{\theScale}{
           $\begin{array}{ccccc}
              \swarrow y	&	\multicolumn{4}{c}{2ih+1}\\ \midrule
              \rightarrow x	&	(i+1)h+(2+t_{i+1})W-8  & (i+1)h+(3+t_{i+1})W-8  & \cdots & (i+1)h+(1+|v|+t_{i+1})W-8
              \\ \toprule
              \textup{Blocks} & \bnCOPYLINEFEED{$(v_0$)}{} & \bnZAGCOPY{$(v_1)$}{} & \cdots & \bnZAGCOPY{$(v_{|v|-1})$}{}
              \\ 
              \midrule
              \textup{Marker}	&	i+2+t_{i+1} &	i+2+t_{i+1} & \cdots& i+2+t_{i+1}
            \end{array}
            $}}\\[4pt]	
        where ${v = u^{1+t_{i+1}} = s\cdot p_{i+1+t_{i+1}}}\neq\epsilon$ (as $s$ and $\alpha^{i+1+t_{i+1}}$ are not both $\epsilon$). 
        This row ends at position $((i+1)h+(1+t_{i+1})W-1,2(i+1)h)$.
      \end{itemize} 
      % 
    \item[$\bullet$ \textup{(Halt 1)} if $u^{1+t_i} = \word0^r1$ and $\alpha^{1+i+t_{i+1}} = \epsilon$:] then $r = t_{i+1}-t_i-1$ and the last rows of the geometrical block configuration consist from left to right of the sequence of geometrical blocks located at the following coordinates:\\[4pt] %, as illustrated in Figure~\ref{fig:final:geom:config:halt:1}: \\[4pt] 
      \centerline{\hspace*{-1.5cm}\scalebox{\theScale}{
          $\begin{array}{ccccccccc}
             \swarrow y	&	\multicolumn{4}{c}{2ih} & & (2i-1)h+1 & & 2(i+1)h
             \\ \cmidrule{1-5} \cmidrule{7-7} \cmidrule{9-9}
             \rightarrow x	&	ih+(1+t_{i})W  & \cdots & ih+(t_{i+1}-1)W & ih+t_{i+1}W & & ih+(1+t_{i+1})W-1&  & (i+1)h+(1+t_{i+1})W
             \\ \toprule
             \textup{Blocks} & \bnREAD{\word0}{} & \cdots & \bnREAD{\word0}{} & \bnREAD{\word1}{} & & \bnRETURNLINEFEED{} & &  \bnHALT
             \\ \midrule
             \textup{Marker}	&	i+1+t_i &	\cdots & i+t_{i+1}-1 & i+t_{i+1}  &&i+1+t_{i+1}  & & i+2+t_{i+1}
           \end{array}
           $}}\\[4pt]	
     \item[$\bullet$ finally, \textup{(Halt 2)} if $u^{1+t_i} = \word0^r$ for some $r\geq0$:] then the $i$-th zig-row is last row of the geometrical block configuration and consists of the sequence of geometrical blocks located at the following coordinates:\\[4pt] %, as illustrated in Figure~\ref{fig:final:geom:config:halt:2}: \\[4pt] 
       \centerline{\hspace*{-1.5cm}\scalebox{\theScale}{
           $\begin{array}{ccccc}
              \swarrow y	&	\multicolumn{4}{c}{2ih} 
              \\ \midrule
              \rightarrow x	&	ih+(1+t_i)W & \cdots & ih+(r+t_{i})W & ih+(1+r+t_{i})W
              \\ \toprule
              \textup{Blocks} & \bnREAD{\word0}{} & \cdots & \bnREAD{\word0}{} & \bnHALT{}
               \\ \midrule
               \textup{Marker}	&	i+1+t_i &	\cdots & i+r+t_i & i+r+1+t_i
            \end{array}
            $}}%\\[4pt]
      \end{description}
    \end{itemize}
\end{lemma}

\begin{corollary}
The read positions and write positions of blocks in consecutive rows are properly aligned.
\end{corollary}


==> block-white.tex <==
%!TEX root =  icalp2018.tex

\begin{figure}
{\setlength{\extrarowheight}{3pt}
$$
\begin{array}{r@{}r@{}r@{\,}r@{\,}r@{\,}r@{\,}r@{\,}rr@{{~~\longrightarrow~~}}c@{~}r@{\,:\,}l}
\pointHere{t_0}&&\pointHere{t_1}&&\pointHere{t_2}&\pointHere{t_3}\\
\cline{2-4}
&\kase{\pQ0\word0}&\kase{\pQ1\word1}&\kase{\word0}&\kase{}&&&&&{\texttt{Append}}&[2]&\word{11}\\[2pt]
\cline{2-6}
&&&\kase{\pQ3\word0}&\kase{\pQ0\word1}&\kase{\word1}&\kase{}&&&
{\texttt{Append}} &[1]&\epsilon\\[2pt]
\cline{4-6}
&&&&&\kase{\pQ2\word1}&\kase{}&&&{\texttt{Append}}&[3]&\word{0}\\
\cline{6-7}
&&&&&&\kase{\pQ0\word0}&\kase{\pQ1}&&{\texttt{Halt}} &[1]&\epsilon\\[2pt]
\cline{7-7}
\end{array}
$$
}%
%
\includegraphics[width=\textwidth]{new-block-simulation-example.pdf}
\end{figure}
%


==> bricks.tex <==
%!TEX root =  icalp2018.tex

%%%%---------------------------------------------------------------
\section{The seed conformation and bricks}
%%%%---------------------------------------------------------------
\label{sec:bricks}

This section presents the exact geometry of each brick. The bead type sequence of each brick are given in the next section. Even if one can recover the bead type sequence from the figures, we believe it easier to have a separated section with all the sequences, for reference or implementation purposes for instance.

This section mainly consists of key figures which explains in full details the exact shape of each brick. 

In this section, we also prove key geometrical lemmas that demonstrate that: (1) all figures presented here are \emph{generic}, i.e. describe faithfully \emph{all} shape possible whatever the SCTS simulated; and (2) all the bricks plug into each other as desired. 

%%%%%%%%%%%%---------------------------------------------------------------
\subparagraph{Notation.}
%%%%%%%%%%%%---------------------------------------------------------------
Given an infinite sequence of directions $(d_i)\in\{\NEb,  \Eb,  \SEb,  \SWb, \Wb, \NWb\}^{\mathbb N}$, and a finite bead type sequence $b\in B^*$, we denote by $\conformation(b, d)$ the conformation $b_0 d_0 b_1 d_1\cdots d_{|b|-2} b_{|b|-1}$ that maps $b$ along the path $d$. We will use the following convenience functions which will ease the description of the bricks:
%
\begin{itemize}     
\item $\Epath(b) = \conformation(b, (\Eb)^\infty)$ and similarly, $\SEpath$, \SWpath$, \Wpath$, $\NWpath$ and $\NEpath$ that map a bead type sequence along the paths $(\SEb)^\infty$, $(\SWb)^\infty$, $(\Wb)^\infty$, $(\NWb)^\infty$, and $(\NEb)^\infty$ respectively.
%
\item $\Eglider(b) = \conformation\left(b, \left(\NEb, \NWb, \Eb, \SEb, \SWb, \Eb\right)^\infty\right)$ 
\item $\Eglider'(b) = \conformation\left(b, \left(\SEb, \SWb, \Eb, \NEb, \NWb, \Eb\right)^\infty\right)$ 
\item $\SERglider(b) = \conformation\left(b, \left(\NEb, \Eb, \SEb, \Wb, \SWb, \SEb \right)^\infty\right)$ 
\item $\NEglider(b) = \conformation\left(b, \left(\NWb, \Wb, \NEb, \Eb, \SEb, \NEb \right)^\infty\right)$ 
\end{itemize}

\clearpage

%%%%%%%%---------------------------------------------------------------
\subsection{The seed conformation}
%%%%%%%%---------------------------------------------------------------

The seed $\ModuleSeed{(u)}$ is a conformation encoding the input dataword $u$ of the simulated SCTS. It is made of 4 types of conformations, (see Figure~\ref{fig:brick:Seed:u} for an illustration):
%
\begin{align*}
%
\SEG{Seed}{Begin} 
&	= 
	{\left(\bJ{8}\SWbond\bJ{7}\,\SWbond\right)^{2+\frac{h-3}{4}}}
	\bJ{11}
	\SWbond\bJ{12}
	\Wbond\bJ{16}
	\Wbond\bJ{17}
	\Wbond\bJ{18}
\\
\SEG{Seed}{Suffix} 
&	= \begin{array}[t]{l}
	\bA9\SWbond
	\bA{12}\Wbond
	\bB0\Wbond
	\bB1\NWbond
	\bB2\Ebond
	\bB3\NEbond
	\bB4\NWbond
	\bC4\NWbond
	\bA0\left(\Wbond\,\bA0\right)^{w-17}\SWbond
	\bH{8}\SWbond
	\\ \quad 
	\bH{19}\SWbond
	\bH{20}\Wbond
	\bH{21}\SWbond
	\bH{24}\Wbond
	\bI{15}\Wbond
	\bI{15}\Wbond
	\bI{16}\Wbond
	\bI{17}\Wbond
	\bI{19}\Wbond
	\bI{19}\Wbond
	\bJ{12}\Wbond
	\\ \quad
	\bJ{16}\Wbond
	\bJ{17}\Wbond
	\bJ{18} 
	\end{array}
\\
\SEG{Seed}{$(\word 0)$} 
&	= 
	\bL{17}\Wbond
	\bL{18}\Wbond
	\bL{47}\SWbond
	\bL{48}\NWbond
	\bL{49}\Wbond
	\bL{82}\Wbond
	\bL{83}\NWbond
	\bA6
\\
\SEG{Seed}{$(\word 1)$} 
&	= 
	\bL{17}\Wbond
	\bL{18}\Wbond
	\bL{48}\Wbond
	\bL{82}\Wbond
	\bL{83}\NWbond
	\bL{84}\Wbond
	\bA6
\\
\SEG{Seed}{End} 
&	= \begin{array}[t]{l}
	\bK{34}\SWbond
	\left(\bK{45}\SWbond\bK{40}\,\SWbond\right)^{11}
	\left(\bK{46}\SWbond\bK{47}\,\SWbond\right)^{k-2}
	\left(\bK{57}\SWbond\bK{52\,\SWbond}\right)^{k-2}
	\\ \quad
	\left(\bK{59}\SWbond\bK{60}\,\SWbond\right)^{k-18}
	\left(\bK{69}\SWbond\bK{64}\,\SWbond\right)^{10}
	\bK{69} \SWbond
	\bM{20} \SEbond
	\bM{26} \SWbond
	\bM{27}
	\\ \quad 
	\Wbond\,
	\bM{28}\SWbond
	\bM{29}\Ebond
	\bM{30}.
	\end{array}
%
\end{align*}

\medskip 

\noindent
Each letter $a\in\{\word0,\word1\}$ is encoded in the seed by the conformation: (note that it heads westwards)
$$
\SEG{Seed}{Letter$(a)$} = \left(\SEG{Seed}{$(\word1)$}\Wbond\SEG{Seed}{Suffix}\,\Wbond\right)^{n-1} 
\SEG{Seed}{$(a)$}\Wbond\SEG{Seed}{Suffix}
$$
\medskip

Then, the conformation $\ModuleSeed{(u)}$ is: (note that it heads southwestwards, see Fig.~\ref{fig:brick:Seed:u})
% 
$$
\ModuleSeed{(u)} = 
\SEG{Seed}{Begin} 
\Wbond
\left(\overset{|u|}{\concat{i=1}} 
  \SEG{Seed}{Letter$(u_{|u|-i})$}
  \,\Wbond
\right)
\SEG{Seed}{End}
$$

This completes the definition of the primary structure of the oritatami system ${\TMO_\TMS=((\pi_\TMS)^\infty,\heart,3)}$ whose folding from the seed configuration \ModuleSeed{(u)} simulates step-by-step the computation of SCTS $\TMS$ starting with input dataword~$u$.  Section~\ref{sec:rule} presents the full description of the attraction rule~$\heart$, completing the description of the oritatami system $\TMO_\TMS$.

\figBrickHereLandscapeSize%
	{Seed-Brick}%
	{The brick $\protect\ModuleSeed{(u)}$.}%
	{fig:brick:Seed:u}%
	{1.075\textheight}%
	{\textwidth}

\clearpage

%%%%%%%%---------------------------------------------------------------
\subsection{The bricks for module A}
%%%%%%%%---------------------------------------------------------------

Module $\ModuleA$ adopts three brick conformations: \AZigUp, \AZigDown, and \AZag, where the two last ones are just obtained by mirroring and rotating the first:
\begin{align*}
\AZigUp 
&	=  \bA0 \Eb \bA1\NWb \bA2 \Eb \bA3 \SEb\bA4 \NEb (\bA5 \NWb \bA6 \Wb \bA7 \NEb \bA8 \Eb \bA9 \SEb \bA{10} \NEb)^{3k-1} \bA5 \NWb \\
& 	\retraitAlign  
	\bA6 \Wb \bA7 \NEb \bA6 \Eb \bA9 \SEb \bA{10} \NEb \bA{11} \NWb \bA{12}
\\[2mm]
\AZigDown 
&	= \mirror(\AZigUp)
\\[1mm]
\AZag 
&	= \rot(\AZigUp)
\end{align*}

\figBrickHere%
	{A-Zig_Init-UPRIGHT}%
	{Module \ModuleA: Brick $\AZigUp$.}%
	{fig:A:brick:ZigUp}%
		
\clearpage
	
%%%%%%%%---------------------------------------------------------------
\subsection{The bricks for module B}
%%%%%%%%---------------------------------------------------------------

Module $\ModuleB$ adopts four brick conformations plus some incomplete ones if the folding stops because the dataword in the simumlated SCTS is empty.

\begin{align*}
\BZigUp 
&	=  \bB0 \Eb \bB1 \SEb \bB2 \Wb \bB3 \SWb \bB4
\\[2mm]
\BZigDown 
&	=  \mirror(\BZigUp)
\\[1mm]
\BZag 
&	=  \rot(\BZigUp)
\\[2mm]
\BHalt 
&	=  \bB0 \Wb \bB1 \SWb \bB2 \SWb \bB3 \SWb \bB4
\end{align*}

\figBrickHere%
	{B-Empty_Word_Tape}%
	{Module \ModuleB: Brick $\BZigUp$.}%
	{fig:B:brick:ZigUp}

\clearpage

	
%%%%%%%%---------------------------------------------------------------
\subsection{The bricks for module C}
%%%%%%%%---------------------------------------------------------------

Module $\ModuleC$ adopts four brick conformations:

\begin{align*}
\CZigUp 
&	= 	(\bC0 \SWb \bC1 \SWb \bC2\, \SWb )^{2k-1} \bC0 \SWb \bC1 \SWb \bC2 \, \Eb 
\\
&		\retraitAlign 
		(\bC3 \NEb \bC4 \NEb \bC5\, \NEb)^{k} \, \bC3 \NEb \bC7 \NEb 
		(\bC8 \NEb \bC6 \NEb \bC7\, \NEb) ^{k-1} \, \bC8 \, \SEb
\\
&		\retraitAlign 
		(\bC9 \SWb \bC{10} \SWb \bC{11} \SWb \bC{12} \SWb \bC{13} \SWb \bC{14} \, \SWb)^{k-1}
		\bC9 \SWb \bC{10} \SWb \bC{15} \SWb \bC{16} \SWb \bC{13}
\\[2mm]
\CZigDown 
&	=  \mirror(\CZigUp)
\\[1mm]
\CZag 
&	=  \rot(\CZigUp)
\\[2mm]
\CEnd
&	=  (\bC0 \NWb \bC1 \NWb \bC2 \, \NWb )^{2k-1} \bC0 \NWb \bC1 \NWb \bC2 \, \Eb 
\\
&		\retraitAlign 
		(\bC3 \NEb \bC4 \NEb \bC5 \, \NEb)^{k} \, \bC3 \, \SEb 	
\\
&		\retraitAlign 
		\bC7 \SWb  \bC8 \SWb (\bC6 \SWb \bC7 \SWb \bC8 \, \SWb ) ^{k-1} \, \bC9 \, \SWb
\\
&		\retraitAlign 
		(\bC{10} \SEb \bC{11} \SEb \bC{12} \SEb \bC{13} \SEb \bC{14} \SEb \bC9 \, \SEb)^{k-1}
		\SEb \bC{10} \SEb \bC{15} \SEb \bC{16} \SEb \bC{13}
\end{align*}

\figBrickHere%
	{C-End_Word_Tape-Upright}%
	{Module \ModuleC: Brick $\CZigUp$.}%
	{fig:C:brick:ZigUp}
	
\figBrickHere%
	{C-End_of_Tape-Expanded}%
	{Module \ModuleC: Brick $\CEnd$.}%
	{fig:C:brick:End}
	
\clearpage
	

%%%%%%%%---------------------------------------------------------------
\subsection{The bricks for the modules D}
%%%%%%%%---------------------------------------------------------------

\paragraph{The zig and zag brick conformations.}

\begin{align*}
\SegDZigUp{0} 
&	= 	\NEpath\!\left(\bbD{23}{33}\conc\bbE{6}{11}\conc(\bbE{0}{11})^{\kappa-1}\right)
\\
\SegDZigUp{1} 
&	=	\SWpath\!\left( (\bbE{12}{23})^{\kappa}\conc \bbD{49}{45} \right)
\\
\SegDZigUp{2} 
&	=	\NEpath\!\left( \bSB{\bbD{34}{44}}\conc \bbE{30}{35}\conc (\bbE{24}{35})^{\kappa-1}\right)
\\
\SegDZigUp{3} 
&	=	\SWpath\!\left( (\bbE{36}{47})^{\kappa}\conc \bbD{54}{50} \right)
\\[2mm]
\DUZigUp{2,0} 
&	= \SegDZigUp{0} \Eb \SegDZigUp{1} \Eb \SegDZigUp{2} \Eb \SegDZigUp{3} \Eb \SegDZigUp{0} \Eb \SegDZigUp{1} 
\\
\DUZigUp{1,0} 
&	= \SegDZigUp{2} \Eb \SegDZigUp{3} \Eb \SegDZigUp{0} \Eb \SegDZigUp{1} \Eb \SegDZigUp{2} \Eb \SegDZigUp{3} 
\\
\DUZigUp{0,0}  
&	= \DUZigUp{2,0}\subst{(\NEpath(\bbD{0}{16})\, \NEb) @0..16}
\\
\DUZigUp{r,1} 
&	= \DUZigUp{r,0}\subst{(\bD{17}\,\SWb )@(3W+22), \SWpath(\bbD{18}{22})@(3W+25)..(3W+29)} 
& 	\text{for $r\in\{0,1,2\}$}
\\
\DZZigUp{r,t} 
&	= \DUZigUp{r,t}\substOpen{(\bL{17} \NEb \bL{18} \, \NEb)@(3w+1..3w+2),}
\\[-2mm]
&	\hspace*{2cm} \substClose{(\NEpath(\bbD{55}{62})\,\NEb)@(3w+6)..(3w+13)}
&	\begin{array}[t]{r} 
		\text{for $r\in\{0,1,2\}$}
		\\
		\text{and $t\in\{0,1\}$}
	\end{array}
\end{align*}
\\
The zig-down and zag brick conformations are obtained by mirroring and rotating the zig-up brick conformation: for $x\in\{\word0,\word1\}$, $r\in\{0,1,2\}$ and $t\in\{0,1\}$, we have 
\begin{align*}
\DxZigDown{x,r,t}
&	= \mirror(\DxZigUp{x,r,t})
\\
\DxZag{x,r,t}
&	= \rot(\DxZigUp{x,r,t})
\end{align*}

%% FIG D

\figBrickHereSize%
	{D-NewLetter-0-Zig}%
	{Modules \ModuleDZ{r,t}: Bricks $\DZZigUp{r,t}$.}%
	{fig:D0:brick:ZigUp}%
	{1.3\textwidth}%
	{\textheight}
\clearpage

\paragraph{The append brick conformations.}

\begin{align*}
\SegDAppend{0} 
&	= 	\Epath(\bbD{23}{27}) \SEb \SEpath(\bbD{28}{30}) \SWb \bD{31} \Eb \bD{32} \NEb \bD{33} \NEb
\\
&	\retraitAlign
		\Eglider'\!\left(\bbE{6}{11}\conc(\bbE{0}{11})^{\kappa-1}\right)
\\
\SegDAppend{1} 
&	=	\Eglider'\!\left( (\bbE{12}{23})^{\kappa}\right) \NWb \Wpath(\bbD{49}{45})
\\
\SegDAppend{2} 
&	= 	\Epath(\bbD{34}{38}) \SEb \SEpath(\bbD{39}{41}) \SWb \bD{42} \Eb \bD{43} \NEb \bD{44} \NEb
\\
&	\retraitAlign
		\Eglider'\!\left(\bbE{30}{35}\conc(\bbE{24}{35})^{\kappa-1}\right)
\\
\SegDAppend{3} 
&	=	\Eglider'\!\left( (\bbE{36}{47})^{\kappa}\right)\NWb \Wpath(\bbD{54}{50})
\\
\SegDAppend{\textit{init}} 
&	=	\bD{0} \Eb \bD{1} \SWb \bD{2} \Eb \bD{3} \SEb \bD{4} \SWb \bD{5} \Eb \bD{6} \NEb \bD{7} \NWb \bD{8} \NWb \bD{9} \NWb \bD{10} \Wb
\\
&	\retraitAlign  \bD{11} \NWb \bD{12} \Eb \bD{13} \Eb \bD{14} \SEb \bD{15} \SEb \bD{16}
\\
\SegDAppend{\textit{end}} 
&	=	\bD{18} \Eb \bD{19} \SEb \bD{20} \SEb \bD{21} \SWb \bD{22}
\\
\SegDAppend{\textit{spike}} 
&	=	\bD{55} \SWb \bD{56} \SEb \bD{57} \NEb \bD{58} \NEb \bD{59} \NEb \bD{60} \SEb \bD{61} \SWb \bD{62}
\\
\\[2mm]
\DUAppend{2,0} 
&	= \SegDAppend{0} \Eb \SegDAppend{1} \NEb \SegDAppend{2} \Eb \SegDAppend{3}
%\\& \hspace*{4cm}	
\NEb \SegDAppend{0} \Eb \SegDAppend{1} 
\\
\DUAppend{1,0} 
&	= \SegDAppend{2} \Eb \SegDAppend{3} \NEb \SegDAppend{0} \Eb \SegDAppend{1}
%\\& \hspace*{4cm} 
\NEb \SegDAppend{2} \Eb \SegDAppend{3} 
\\
\DUAppend{0,0}  
&	= \DUAppend{2,0}\subst{(\SegDAppend{\textit{init}}\, \SEb) @0..16}
\\
\DUAppend{r,1} 
&	= \DUAppend{r,0}\substOpen{(\bD{17}\,\NEb )@(3W+22),}
\\[-2mm]
&	\hspace*{2.9cm} \substClose{(\NWb \SegDAppend{\textit{end}})@(3W+25)..(3W+29)} 
	\quad \text{for $r\in\{0,1,2\}$}
\\
\DZAppend{r,t} 
&	= \DUAppend{r,t}\substOpen{(\bL{17} \Eb \bL{18} \, \NEb)@(3w+1..3w+2),}
\\[-2mm]
&	\hspace*{2.9cm} \substClose{(\SegDAppend{\textit{spike}} \,\Eb)@(3w+6)..(3w+13)}
	\quad
	\begin{array}[t]{r} 
		\text{for $r\in\{0,1,2\}$}
		\\
		\text{and $t\in\{0,1\}$}
	\end{array}
\end{align*}

\begin{sidewaysfigure}
  \subfigBrickLandscape{D-NewLetter0-0-Expanded.pdf}%D-Letter-0-1-Expanded.pdf}%
    {The brick $\DZAppend{0,0}$.}%
    {fig:D:brick:000:Append}
  \subfigBrickLandscape{D-NewLetter0-1-Expanded.pdf}%D-Letter-1-1-Expanded.pdf}%
    {The brick $\DZAppend{1,0}$.}%
    {fig:D:brick:010:Append}
  \subfigBrickLandscape{D-NewLetter0-2-Expanded.pdf}%
    {The brick $\DZAppend{2,0}$.}%
    {fig:D:brick:020:Append}

  \subfigBrickLandscape{D-NewLetter0-0Last-Expanded.pdf}%
    {The brick $\DZAppend{0,1}$.}%
    {fig:D:brick:001:Append}
  \subfigBrickLandscape{D-NewLetter0-1Last-Expanded.pdf}%
    {The brick $\DZAppend{1,1}$.}%
    {fig:D:brick:021:Append}
  \subfigBrickLandscape{D-NewLetter0-2Last-Expanded.pdf}%
    {The brick $\DZAppend{2,1}$.}%
    {fig:D:brick:021:Append}

  \caption{Module $\ModuleDZ{r,t}$: Bricks $\DWrite$.}
  \label{fig:brick:D:write}
\end{sidewaysfigure}
	
\clearpage
	
%%%%%%%%---------------------------------------------------------------
\subsection{The bricks for the modules E}
%%%%%%%%---------------------------------------------------------------

%%%%%%%%%%%%---------------------------------------------------------------
\paragraph{Zig-up, zig-down and zag bricks.}
%%%%%%%%%%%%---------------------------------------------------------------

\begin{align*}
\SEGE{A\ZigUp} 
&	= \Bigl(\NEpath\bigl((\bbF{0}{11})^\kappa\bigr) \Eb 
		 \SWpath\bigl((\bbF{12}{23})^\kappa\bigr) \Eb
\\[-2mm]	&	\retraitAlign
		\NEpath\bigl((\bbF{24}{35})^\kappa\bigr) 
		\Eb \SWpath\bigl((\bbF{36}{47})^\kappa\bigr)\Bigr)^\infty
\\
\SEGE{B\ZigUp} 
&	= \Bigl(\NEpath\bigl(\bbG{0}{11})^\kappa\bigr) \Eb 
		\SWpath\bigl((\bbG{12}{23})^\kappa\bigr) \Eb
\\[-2mm]	&	\retraitAlign
		 \NEpath\bigl((\bbG{24}{35})^\kappa\bigr) \Eb
		 \SWpath\bigl((\bbG{36}{47})^\kappa\bigr)\Bigr)^\infty
\\
\HEAD{E$_a$\ZigUp} 
&	= \SEGE{A\ZigUp}_{b..b+3c(a)-2} ~ d ~ \bS{\bF{51}} ~ d ~ \SEGE{B\ZigUp}_{b+3c(a)..b+K-2}
&	\begin{array}[t]{r} 
		\makebox[1cm][r]{\text{\quad where $b= 0$ if $a$ is even,}}
		\\ 
		\makebox[1cm][r]{\text{and $b=2\lambda$ if $a$ is odd;}}
		\\
		\makebox[1cm][r]{\text{and $d = \NEb$ if $\lfloor\frac{3c-2}{\lambda}\rfloor$ is even, else $d=\SWb$}}  
		\end{array}
\\[2mm]
\SEGE{C\ZigUp} 
&	= \bH{0} \Eb \bH{1} \NWb \bH{2} \Eb \bH{3} \SEb \bH{4} \NEb 
\\	&	\retraitAlign
		\NEglider\bigl((\bbH{5}{16})^{q-1} \conc \bbH{5}{10} \conc \bbH{17}{22}\bigr)
		\NEb \bH{23} \NWb \bH{24}
\\
\SEGE{D$_0$\ZigUp}
&	= \bI{15} \SEb \SWpath\bigl(\bbI{1}{5} \conc (\bbI{0}{5})^{k-1} \conc \bbI{0}{1} \conc \bI{18}\bigr)
\\
\SEGE{D$_1$\ZigUp} 
&	= \NEpath\bigl(\bI{19} \conc \bbI{7}{8} \conc (\bbI{6}{8})^{2k-1}\conc \bbI{6}{7}\bigr) \NWb \bI{15} \Eb \bI{16}
\\
\SEGE{D$_2$\ZigUp}
&	= \SWpath\bigl(\bI{17}\conc \bbI{10}{11} \conc (\bbI{9}{11})^{2k-1} \conc \bbI{9}{10}\conc \bI{19}\bigr)
\\
\SEGE{D$_3$\ZigUp}
&	= \NEpath\bigl(\bI{18} \conc \bbI{13}{14} \conc (\bbI{12}{14})^{2k-1} \conc \bbI{12}{13} \conc \bI{19}\bigr)
\\
\SEGE{D$_4$\ZigUp}
&	= \SWpath\bigl(\bI{19} \conc \bbI{1}{2} \conc (\bbI{0}{2})^{2k}\bigr)
\\
\TAIL{E\ZigUp} 
&	= \SEGE{C\ZigUp} \Eb \SEGE{D$_0$\ZigUp} \Eb \SEGE{D$_1$\ZigUp} \Eb \SEGE{D$_2$\ZigUp} \Eb \SEGE{D$_3$\ZigUp} \Eb \SEGE{D$_4$\ZigUp}
\\[2mm]
\EaZigUp{0} 
&	= \HEAD{E$_0$\ZigUp}\subst{(\bF{48}\NEb \bF{49}\,\NEb)@0..1, (\bF{50}\,\NEb)@11} \SWb \bG{48} 
		\Eb \TAIL{E\ZigUp}
\\
\EaZigUp{a>0} 
&	= \HEAD{E$_{a}$\ZigUp}\SWb \bG{48} \Eb \TAIL{E\ZigUp}
\\[2mm]
\EaZigDown{a\geq 0} 
&	= \mirror(\EaZigUp{a})
\\
\EaZag{a\geq 0} 
&	= \rot(\EaZigUp{a})
\end{align*}


\begin{sidewaysfigure}[h]
  %
  \begin{subfigure}{\textheight}
    \centering
    \adjustbox{max size= {\textheight}{.4\textwidth}}{
    \begin{tikzpicture}
    \node () at (0,0){\includegraphics[width=15cm,height=15cm,keepaspectratio]{ModulesDescriptions/E-Padding-Outline-Up.pdf}};
%
%\foreach \x in {-10,...,10}
%      \draw (\x cm, -10cm)--(\x cm, 10cm) (-10 cm, \x cm)--(10 cm, \x cm) ;
%\draw [draw=red] (0, -10cm)--(0 cm, 10cm) (-10 cm, 0 cm)--(10 cm, 0 cm) ;
%
    \node () at (-3.5cm,-1cm) {\small\begin{tabular}{c} Segment $\SEGE{A}$\\ folded as brick $\SEGE{A\ZigUp}$\end{tabular}};
%
    \node () at (0.3cm,-1cm) {\small\begin{tabular}{c} Segment $\SEGE{B}$\\ folded as brick $\SEGE{B\ZigUp}$\end{tabular}};
%
    \node () at (2.65cm,2cm) {\small\begin{tabular}{r} Segment $\SEGE{C}$\\ folded as brick $\SEGE{C\ZigUp}$\hspace*{2.5mm}\end{tabular}};
%
    \node [anchor=west] () at (4cm,0cm) {\small\begin{tabular}{l} \hspace*{2.5mm} Segment $\SEGE{D\ensuremath{_{0..4}}}$\\ folded as brick $\SEGE{D\ensuremath{_{0..4}}\ZigUp}$\end{tabular}};
%
    \end{tikzpicture}
    }
    \caption{Module $\ModuleE$: Blueprint of the brick $\EaZigUp{a}$.}
    \label{fig:brick:E:upright:outline}
  \end{subfigure}
  %
  \begin{subfigure}{\textheight}
    \hspace*{-1cm}\adjustbox{max size= {1.075\textheight}{.6\textwidth}}{
    \begin{tikzpicture}
    \node () at (0,0){\includegraphics[scale=1.25]{ModulesDescriptions/E-Padding-All-Zig-Up.pdf}};
%
%\foreach \x in {-20,...,20}
 %     \draw (\x cm, -10cm)--(\x cm, 10cm) (-10 cm, \x cm)--(10 cm, \x cm) ;
%\draw [draw=red] (0, -10cm)--(0 cm, 10cm) (-10 cm, 0 cm)--(10 cm, 0 cm) ;
%
    \node () at (-16.5cm,-6.75cm) {\small\begin{tabular}{c} Beginning of brick $\SEGE{A\ZigUp}$\end{tabular}};
%
    \node () at (-10cm,-6.25cm) {\small\begin{tabular}{c} Repeated\\bond pattern\\ inside brick $\SEGE{A\ZigUp}$\end{tabular}};
%
    \node () at (-2.75cm,-6.5cm) {\small\begin{tabular}{r} Junction between bricks $\SEGE{A\ZigUp}$ and $\SEGE{B\ZigUp}$\end{tabular}};
%
    \node () at (4.5cm,-6.25cm) {\small\begin{tabular}{c} Repeated\\bond pattern\\ inside brick $\SEGE{B\ZigUp}$\end{tabular}};
%
    \node () at (9.5cm,-6.5cm) {\small\begin{tabular}{r} Bricks $\SEGE{C\ZigUp}$ and $\SEGE{D\ZigUp}$\end{tabular}};
%
    \end{tikzpicture}
    }
    \caption{Precise description of the brick $\EaZigUp{a}$.}
    \label{fig:brick:E:upright:details}
  \end{subfigure}
  %
  \caption{Module $\ModuleEa{a}$: Bricks $\EaZigUp{a}$.}
  \label{fig:brick:E:upright}
\end{sidewaysfigure}

\clearpage


%%%%%%%%%%%%---------------------------------------------------------------
\paragraph{Carriage-return bricks.}
%%%%%%%%%%%%---------------------------------------------------------------

\begin{align*}
\SEGE{A\bZigZag} 
&	= \Eglider\bigl(\SEGE{A}\bigr)
\\
\SEGE{B\bZigZag} 
&	= \Wpath\bigl(\SEGE{B}\bigr)
\\
\HEAD{E$_a$\bZigZag} 
&	= \SEGE{A\bZigZag}_{b..b+3c(a)-2} \SWb \bF{51} \SEb \SEGE{B\bZigZag}_{b+3c(a)..b+K-2}
&	\begin{array}[t]{r} 
		\makebox[0em][r]{\text{\quad where $b= 0$ if $a$ is even,}}
		\\ 
		\makebox[0em][r]{\text{and $b=2\lambda$ if $a$ is odd;}}
		\end{array}
\\[2mm]
\SEGE{C\bZigZag} 
&	= \Wpath\bigl(\bbH{0}{4} \conc (\bbH{5}{16})^{q-1} \conc \bbH{5}{10} \conc \bbH{17}{19}\bigr)
		\SEb \bH{20} \Eb \bH{21} \Eb \bH{22} \SWb \bH{23} \Wb \bH{24}
\\
\SEGE{D$_0$\bZigZag}
&	= \bI{15} \NWb \bI{1} \NWb \Wpath\bigl( \bbI{2}{5} \conc (\bbI{0}{5})^{k-1} \conc \bbI{0}{1}\bigr)
		\SEb \bI{18}
\\
\SEGE{D$_1$\bZigZag} 
&	= \bI{19} \NWb \Wpath\bigl(\bbI{7}{8} \conc (\bbI{6}{8})^{2k-1}\conc \bbI{6}{7}\bigr) \SEb \bI{15} \Wb \bI{16}
\\
\SEGE{D$_2$\bZigZag}
&	= \bI{17}\NEb \Wpath\bigl(\bbI{10}{11} \conc (\bbI{9}{11})^{2k-1} \conc \bbI{9}{10}\bigr) \SEb \bI{19}
\\
\SEGE{D$_3$\bZigZag}
&	= \bI{18}  \NWb \Wpath\bigl(\bbI{13}{14} \conc (\bbI{12}{14})^{2k-1} \conc \bbI{12}{13}\bigr) \SWb \bI{19}
\\
\SEGE{D$_4$\bZigZag}
&	= \bI{19} \NEb \Wpath\bigl(\bbI{1}{2} \conc (\bbI{0}{2})^{2k}\bigr)
\\
\TAIL{E\bZigZag} 
&	= \SEGE{C\bZigZag} \Wb \SEGE{D$_0$\bZigZag} \Wb \SEGE{D$_1$\bZigZag} \Wb \SEGE{D$_2$\bZigZag} \Wb \SEGE{D$_3$\bZigZag} \Wb \SEGE{D$_4$\bZigZag}
\\[2mm]
\EaCR{0} 
&	= \HEAD{E$_0$\bZigZag}\subst{(\bF{48}\Eb \bF{49}\,\SWb)@0..1, (\bF{50}\,\Eb)@11} \Wb \bG{48} 
		\Wb \TAIL{E\bZigZag}
\\
\EaCR{a>0} 
&	= \HEAD{E$_{a}$\bZigZag}\Wb \bG{48} \Wb \TAIL{E\bZigZag}
\end{align*}

\begin{figure}[h]
	\newSubFigBrick%
		{E-Padding-Outline0.pdf}% PDF
		{Blueprint of brick $\EaCR{a=0}$, made of four bricks $\SEGE{A\bZigZag}$, $\SEGE{B\bZigZag}$, $\SEGE{C\bZigZag}$ and $\SEGE{D\bZigZag}$.}% caption
		{fig:brick:schema:EL:CR}% label
		{\textwidth}% width
		{%
			\nodeLabel{0}{0.8}{c}{Segment $\SEGE{A}$ folded as brick $\SEGE{A\bZigZag}$ (when $a=0$)}
			\nodeLabel{-2.45}{-1}{c}{Segment $\SEGE{D\ensuremath{_{0..4}}}$ folded as brick $\SEGE{D\ensuremath{_{0..4}}\bZigZag}$}
			\nodeLabel{2.2}{-1}{c}{Brick $\SEGE{C\bZigZag}$}
			\nodeLabel{5.3}{-1}{c}{Brick $\SEGE{B\bZigZag}$}
		}% node labels
		{} %grid

	\newSubFigBrick%
		{E-Padding-Outline1.pdf}% PDF
		{Blueprint of brick $\EaCR{a>0}$, made of four  bricks $\SEGE{A\bZigZag}$, $\SEGE{B\bZigZag}$, $\SEGE{C\bZigZag}$ and $\SEGE{D\bZigZag}$.}% caption
		{fig:brick:schema:Ea<L:CR}% label
		{\textwidth}% width
		{%
			\nodeLabel{0}{0.8}{c}{Segment $\SEGE{A}$ folded as brick $\SEGE{A\bZigZag}$ (when $a>0$)}
			\nodeLabel{-2.4}{-0.95}{c}{Segment $\SEGE{D\ensuremath{_{0..4}}}$ folded as brick $\SEGE{D\ensuremath{_{0..4}}\bZigZag}$}
			\nodeLabel{2.2}{-0.95}{c}{Brick $\SEGE{C\bZigZag}$}
			\nodeLabel{5.3}{-0.95}{c}{Brick $\SEGE{B\bZigZag}$}
		}% node labels
		{} %grid
		
  \caption{Outline of the four different parts of module $\ModuleEa{a}$, when folded at the end of the appended appendant. See Figure~\ref{fig:brick:E:CR} for the detailed beads of each part.}
  \label{fig:E-outline}
\end{figure}

\begin{figure}[h]
  \subfigBrickPortrait{E-Padding-EA0.pdf}%
  {The $\SEGE{A}$-part of brick \HEAD{E$_{a=0}$\bZigZag}, when $a=0$.}%
  {fig:brick:EA0:CR}

  \subfigBrickPortrait{E-Padding-EA1.pdf}%
  {The $\SEGE{A}$-part of brick $\HEAD{E$_a$\bZigZag}$, when $a$ is odd.}%
  {fig:brick:EA1:CR}

  \subfigBrickPortrait{E-Padding-EA2.pdf}%
  {The $\SEGE{A}$-part of brick $\HEAD{E$_{a>0}$\bZigZag}$, when $a$ is even and positive.}%
  {fig:brick:EA2:CR}

  \subfigBrickPortrait{E-Padding-EB.pdf}%
  {The $\SEGE{B}$-part of brick $\HEAD{E$_a$\bZigZag}$.}%
  {fig:brick:EB:CR}\\[1mm]

  \subfigBrickPortrait{E-Padding-EC.pdf}%
  {The brick $\SEGE{C\bZigZag}$.}%
  {fig:brick:EC:CR}

  \subfigBrickPortrait{E-Padding-ED.pdf}%
  {The brick $\SEGE{D$_{0..4}$\bZigZag}$.}%
  {fig:brick:ED:CR}
  \caption{The bricks $\EaCR{a}$.}
  \label{fig:brick:E:CR}
\end{figure}

\clearpage

%%%%---------------------------------------------------------------
\subsection{The bricks for the modules F}
%%%%---------------------------------------------------------------

Module $\ModuleF$ adopts three brick conformations: zig-up $\FZigUp$, zig-down $\FZigDown$, and zag $\FZag$. the two last are obtained by mirroring and rotating the first.
%
\begin{align*}
\HEAD{F\ZigUp} 
&	= \bJ0 \Eb \bJ1\NWb \bJ2 \Eb \bJ3 \SEb\bJ4 \NEb \NEglider\left((\bbJ{5}{10})^{3k-1}\right)
	 	\NEb \bJ{5} \NWb \bJ{6} \Wb \bJ{7} \NEb
\\	&	\retraitAlign
		 \bJ{11} \NEb \bJ{12} \SEb \bJ{13} \SEb \bJ{14}
		\NEb \bJ{15} \NWb \bJ{16}  \Eb \bJ{17} \Eb \SWpath(\bbJ{18}{23})
\\
\TAIL{F\ZigUp} 
&	= \SWpath(\bJ{48} \conc (\bbJ{51}{48})^{9} \conc \bJ{51} \conc \bJ{52} \conc \bbJ{49}{48})
\\[2mm]
\text{Recall that } \SEG{Exp}{F} 
&	= \concat{i\geq2}  \SEG{Exp$(i)$}{}
\\%[2mm]
\FZigUp 
&	= \HEAD{F\ZigUp} \, \SWb \, \SWpath\!\left(\bbJ{39}{41}\conc \SEG{Exp}{F}_{0..(h-51)}\right)^R \, \SWb  \, \TAIL{F\ZigUp}
\\[2mm]
\FZigDown 
&	= \mirror(\FZigUp)
\\[1mm]
\FZag 
&	= \rot(\FZigUp)
\end{align*}

\figBrickHereSize%
	{F-Zag_init-Upright}%
	{Module \ModuleF: Brick $\FZigUp$.}%
	{fig:F:brick:ZigUp}
	{1.3\textwidth}
	{\textheight}
	
\clearpage


%%%%%%%%---------------------------------------------------------------
\subsection{The bricks for the modules G}
%%%%%%%%---------------------------------------------------------------

%%%%%%%%%%%%---------------------------------------------------------------
\paragraph{Zig-up bricks}
%%%%%%%%%%%%---------------------------------------------------------------

$\ModuleG$ adopts two different bricks in zig-up phase, depending on the letter encoded in the zag-phase above: $\GReadZ$ and $\GReadU$.

%%%
%%% G-READ0
%%%

\subparagraph{The $\protect\GReadZ$ brick.} ~

\begin{align*}
\SEG{G1Start\ZigUp}{Read} 
&	= \bL{0} \Wb \bL{1} \Wb \bL{2} \SEb \bL{3} \Eb \bL{4} \Eb \bL{5} \NEb \bL{6} \NEb \bK3
\\
\SEG{G1GliderNE\ZigUp}{Read} 
&	=  \begin{array}[t]{@{}l@{}l@{}}
		\NEpath\Bigl((\bbK{0}{3})^9 \conc \bbK{0}{2}\Bigr) \Eb \bL{7}\NWb \bL{8} \Eb \bL{9} \SEb \bL{10} 
		\NEb 
		\\ \retraitAlign
		\NEglider\Bigl(\SEG{Exp}{G}_{8..h-51} \conc \bbL{11}{23}\Bigr)
		\end{array} 
\\
\SEG{G2GliderNE\ZigUp}{Read} 
&	= \NEglider\bigl(\bL{24} \conc \bbK{32}{33}\conc (\bbK{28}{33})^{k-3} \conc \bbK{28}{32} \conc \bbL{25}{34}\bigr)
\\
\SEG{G3GliderNE\ZigUp}{Read} 
&	= \NEglider\bigl(\bbL{35}{38} \conc \bbK{35}{39} \conc (\bbK{34}{39})^{k-14}\conc \bK{34}\conc \bK{35} \conc \bL{39}\bigr)
\\[1mm]
\BigSEG{G1..3GliderNE\ZigUp}{Read} 
&	= \SEG{G1GliderNE\ZigUp}{Read} \NEb  \SEG{G2GliderNE\ZigUp}{Read} \NEb \SEG{G3GliderNE\ZigUp}{Read}
\\[3mm]
\SEG{G3GliderSE\ZigUp}{Read\word0} 
&	= \SERglider\bigl(\bbL{40}{41} \conc \bK{45} \conc (\bbK{40}{45})^{10} \conc
		  \bbK{40}{41}\conc \bL{42}\bigr)
\\
\SEG{G3SockNW\ZigUp}{Read\word0} 
&	= \NWpath(\bbL{43}{48}) \SWb \SEpath(\bbL{49}{54}) \Eb \bL{55}
\\
\SEG{G4GliderSE\ZigUp}{Read\word0}
&	= \SERglider\bigl(\bbK{50}{51} \conc  (\bbK{46}{51})^{k-3}\conc \bbK{46}{48} \conc \bL{56}\bigr)
\\
\SEG{G4SockNW\ZigUp}{Read\word0}
&	= \NWpath(\bbL{57}{64}) \SWb \SEpath(\bbL{65}{72}) \Eb \bL{73} 
\\
\SEG{G5GliderSE\ZigUp}{Read\word0}
&	=  \begin{array}[t]{@{}l@{}l@{}}
		\SERglider\Bigl(& 
		\bbK{55}{57} \conc (\bbK{52}{57})^{k-6} \conc \bbK{52}{53} \conc \bbL{74}{75}  \conc \bbK{56}{57} \, \conc
		\\
		& (\bbK{52}{57})^2 \conc \bbK{52}{53} \conc \bL{76} \Bigr)
		\end{array}
\\
\SEG{G5SockNW\ZigUp}{Read\word0}
&	= \NWpath(\bbL{77}{82}) \Wb \SEpath(\bbL{83}{89}) \Eb \bL{90} 
\\
\SEG{G6AGliderSE\ZigUp}{Read\word0} 
&	= \SERglider\bigl(\bK{63}\conc (\bbK{58}{63})^{k-19} \conc \bbK{58}{61} \conc \bL{91}\bigr)
\\
\SEG{G6SockNW\ZigUp}{Read\word0}
&	= \NWpath(\bbL{92}{99} \conc \bbM{0}{4}) \Wb \SEpath(\bbM{5}{18}) \Eb \bM{19} 
\\
\SEG{G6BGlider\ZigUp}{Read\word0} 
&	= \SERglider\bigl(\bbK{67}{69} \conc (\bbK{64}{69})^{10} \conc \bbM{20}{22}\bigr) \SEb 
		\bM{23}
\\
\SEG{G6End\ZigUp}{Read\word0} 
&	= \bM{24} \Eb \bM{25} \Eb \bM{26} \SWb \bM{27} \Wb \bM{28} \SWb \bM{29} \Eb \bM{30}
\\[2mm]
\GReadZ 
&	= \SEG{G1Start\ZigUp}{Read} \NEb \BigSEG{G1..3GliderNE\ZigUp}{Read} 
		\Eb \SEG{G3GliderSE\ZigUp}{Read\word0} \, \Wb  
\\	&	\retraitAlign
		 \SEG{G3SockNW\ZigUp}{Read\word0} \Eb 
		 \SEG{G4GliderSE\ZigUp}{Read\word0} \Wb
		  \SEG{G4SockNW\ZigUp}{Read\word0}\, \Eb 
\\	&	\retraitAlign 
		\SEG{G5GliderSE\ZigUp}{Read\word0}  \Wb 
		 \SEG{G5SockNW\ZigUp}{Read\word0} \Eb
		\SEG{G6AGliderSE\ZigUp}{Read\word0} \,\Wb 
\\	&	\retraitAlign
		\SEG{G6SockNW\ZigUp}{Read\word0} \Eb 
		\SEG{G6BGlider\ZigUp}{Read\word0} \NEb 
		\SEG{G6End\ZigUp}{Read\word0}
\end{align*}

\figBrickHereSize%
	{G-Read_0}%
	{Module \ModuleG: Brick $\GReadZ$.}%
	{fig:G:brick:Read0}%
	{1.35\textwidth}%
	{\textheight}
	
\clearpage

%%%
%%% G-READ1
%%%

\subparagraph{The $\protect\GReadU$ brick.} ~

\begin{align*}
\SEG{G3GliderE\ZigUp}{Read\word1} 
&	= \bL{41} \NWb \bK{45} \Eb \Eglider'\bigl((\bbK{40}{45})^{10}\bigr) 
		\Eb \bK{40} \SEb \bK{41} \SWb \bL{42}
\\
\SEG{G3SockW\ZigUp}{Read\word1} 
&	= \Wpath(\bbL{43}{48}) \SEb \Epath(\bbL{49}{54}) \NEb \bL{55}
\\
\SEG{G4GliderE\ZigUp}{Read\word1}
&	= \Eglider\bigl(\bbK{50}{51} \conc  (\bbK{46}{51})^{k-3}\conc \bbK{46}{48} \conc \bL{56}\bigr)
\\
\SEG{G4SockW\ZigUp}{Read\word1}
&	= \Wpath(\bbL{57}{64}) \SEb \Epath(\bbL{65}{72}) \NEb \bL{73} 
\\
\SEG{G5GliderE\ZigUp}{Read\word1}
&	=  \begin{array}[t]{@{}l@{}l@{}}
		\Eglider\Bigl(& 
			\bbK{55}{57} \conc (\bbK{52}{57})^{k-6} \conc \bbK{52}{53} \conc \bbL{74}{75}  \conc \bbK{56}{57} \, \conc
		\\ 
			&\retraitAlign (\bbK{52}{57})^2 \conc \bbK{52}{53} \conc \bL{76} \Bigr)
		\end{array}
\\
\SEG{G5SockW\ZigUp}{Read\word1}
&	= \Wpath(\bbL{77}{82}) \SWb \Epath(\bbL{83}{89}) \NEb \bL{90} 
\\
\SEG{G6AGliderE\ZigUp}{Read\word1} 
&	= \Eglider\bigl(\bK{63}\conc (\bbK{58}{63})^{k-19} \conc \bbK{58}{61} \conc \bL{91}\bigr)
\\
\SEG{G6SockW\ZigUp}{Read\word1}
&	= \Wpath(\bbL{92}{99} \conc \bbM{0}{4}) \SWb \Epath(\bbM{5}{18}) \NEb \bM{19} 
\\
\SEG{G6BGliderE\ZigUp}{Read\word1} 
&	= \Eglider\bigl(\bbK{67}{69} \conc (\bbK{64}{69})^9 \conc \bbK{64}{66}\bigr) \Eb \bK{67} \NEb 
		\bK{68} \NWb \bK{69}
\\[2mm]
\BigSEG{G3..6GliderE\ZigUp}{Read\word1}
&	=	\SEG{G3GliderE\ZigUp}{Read\word1} \SWb
		\SEG{G3SockW\ZigUp}{Read\word1} \NEb
		\SEG{G4GliderE\ZigUp}{Read\word1}\SWb
\\	&	\retraitAlign
		\SEG{G4SockW\ZigUp}{Read\word1}\NEb
		\SEG{G5GliderE\ZigUp}{Read\word1}\SWb
		\SEG{G5SockW\ZigUp}{Read\word1}\NEb
\\	&	\retraitAlign
		\SEG{G6AGliderE\ZigUp}{Read\word1} \SWb
		\SEG{G6SockW\ZigUp}{Read\word1} \NEb
		\SEG{G6BGliderE\ZigUp}{Read\word1} 
\\[3mm]
\SEG{G6End\ZigUp}{Read\word1} 
&	= \Epath(\bbM{20}{22}) \SEb \Wpath(\bbM{23}{25}) \SWb \Epath(\bbM{26}{29}) \NEb \bM{30}
\\[2mm]
\GReadU 
&	= \SEG{G1Start\ZigUp}{Read} \NEb 
		\BigSEG{G1..3GliderNE\ZigUp}{Read} \SEb \bL{40} \NEb 
\\	&	\retraitAlign
		\BigSEG{G3..6GliderE\ZigUp}{Read\word1} \Eb
		 \SEG{G6End\ZigUp}{Read\word1}
\end{align*}

\figBrickHereLandscapeSize%
	{G-Read_1}%
	{Module \ModuleG: Brick $\GReadU$.}%
	{fig:G:brick:Read1}%
	{1.1\textheight}%
	{1.3\textwidth}
	
\clearpage


%%%%%%%%%%%%---------------------------------------------------------------
\paragraph{Zig-down and Zag: Copy letter \word0\/ and \word1.}
%%%%%%%%%%%%---------------------------------------------------------------

\begin{align*}
\SEG{G1\ZigDown}{Copy} 
&	= \SEpath\bigl(\bbL{0}{6} \conc \bK3 \conc (\bbK{0}{3})^9 \conc \bbK{0}{2} \conc \bbL{7}{10} \conc \SEG{Exp}{G}_{8..h-51} \conc \bbL{11}{17}\bigr) 
\\
\SEG{G2\ZigDown}{Copy} 
&	= \NWpath\bigl(\bbL{18}{24} \conc \bbK{32}{33}\conc (\bbK{28}{33})^{k-3} \conc \bbK{28}{32} \conc \bbL{25}{30}\bigr)
\\
\SEG{G3\ZigDown}{Copy} 
&	= \begin{array}[t]{@{}l@{}l@{}}
		\SEpath\bigl(&\bbL{32}{38} \conc \bbK{35}{39} \conc (\bbK{34}{39})^{k-14}\conc \bbK{34}{35} \conc \bbL{39}{41} \conc \bK{45} \conc 
		\\	
		&(\bbK{40}{45})^{10} \conc \bbK{40}{41}\conc \bbL{42}{48}\bigr)
		\end{array}
\\
\SEG{G4\ZigDown}{Copy} 
&	= \NWpath\bigl(\bbL{49}{55}\conc \bbK{50}{51} \conc  (\bbK{46}{51})^{k-3}\conc \bbK{46}{48} \conc \bbL{56}{63}\bigr)
\\
\SEG{G5\ZigDown}{Copy}
&	= \begin{array}[t]{@{}l@{}l@{}}
		\SEpath(&\bbL{66}{73}\conc \bbK{55}{57} \conc (\bbK{52}{57})^{k-6} \conc \bbK{52}{53} \conc \bbL{74}{75}  \conc \bbK{56}{57}\conc
		\\ 
	 	&	(\bbK{52}{57})^2 \conc \bbK{52}{53} \conc \bbL{76}{81}\bigr)
		\end{array}
\\
\SEG{G6\ZigDown}{Copy} 
&	= \begin{array}[t]{@{}l@{}l@{}}
		\NWpath\Bigl(&\bbL{84}{90}\conc \bK{63}\conc (\bbK{58}{63})^{k-19} \conc \bbK{58}{61} \conc \bbL{91}{99} \conc \bbM{0}{19} \, \conc\\
		& \bbK{67}{69} \conc (\bbK{64}{69})^{10} \conc \bbM{20}{30}\Bigr)
	\end{array}
\\[2mm]
\GZigCopyZ 
&	= \begin{array}[t]{@{}l@{}l@{}}
		\SEG{G1\ZigDown}{Copy} \Eb  \SEG{G2\ZigUp}{Copy} \NEb \bL{31} \SEb  
		\SEG{G3\ZigDown}{Copy} \NEb \SEG{G4\ZigDown}{Copy} \NEb \bL{64} \Eb \bL{65} \, \SWb
		\\[1mm] \retraitAlign
		\SEG{G5\ZigDown}{Copy} \SEb \bL{82} \Eb  \bL{83} \NWb \SEG{G6\ZigDown}{Copy}
		\end{array}
\\
\GZigCopyU 
&	= \begin{array}[t]{@{}l@{}l@{}}
		\SEG{G1\ZigDown}{Copy} \Eb  \SEG{G2\ZigUp}{Copy} \NWb \bL{31} \Eb  
		\SEG{G3\ZigDown}{Copy} \NEb \SEG{G4\ZigDown}{Copy} \Eb \bL{64} \Eb \bL{65} \, \SWb
		\\[1mm] \retraitAlign
		\SEG{G5\ZigDown}{Copy} \SWb \bL{82} \Eb  \bL{83} \NEb  \SEG{G6\ZigDown}{Copy}
	\end{array}
\\[2mm]
\GZagCopyZ
&	= \vmirror\bigl(\GZigCopyZ\bigr) 
\\
\GZagCopyU
&	= \vmirror\bigl(\GZigCopyU\bigr) 
\end{align*}

\figBrickHereSize%
	{G-Copy_0-Zig}%
	{Module \ModuleG: Brick $\GZigCopyZ$.}%
	{fig:G:brick:ZigCopy0}%
	{1.3\textwidth}%
	{\textheight}

\figBrickHereSize%
	{G-Copy_1-Zig}%
	{Module \ModuleG: Brick $\GZigCopyU$.}%
	{fig:G:brick:ZigCopy1}%
	{1.3\textwidth}%
	{\textheight}
	
\clearpage


%%%%%%%%%%%%---------------------------------------------------------------
\paragraph{Line feed brick.}
%%%%%%%%%%%%---------------------------------------------------------------

\begin{align*}
\SEG{G1A\bZagZig}{LF} 
&	= \NWpath(\bbL{0}{3}) \Wb \SEpath(\bbL{4}{6} \conc \bK{3})
\\
\GLF 
&	= \begin{array}[t]{@{}l}
		\SEG{G1A\bZagZig}{LF} \SWb 
		\rot\bigl(\BigSEG{G1..3GliderNE\ZigUp}{Read} \bigr) 
		\SWb \bL{40} \SEb
		\\ \retraitAlign
		\rotateClockwiseAA{\BigSEG{G3..6GliderE\ZigUp}{Read\word1}}
		\SWb \bM{20} \Wb \bM{21} \NWb \bM{22} 
		\\ \retraitAlign
		\SWb \bM{23} \SEb \SEG{G6End\ZigUp}{Read\word0}
	\end{array}
\end{align*}

\figBrickHereSize%
	{G-Line_Feed}%
	{Module \ModuleG: Brick $\GLF$.}%
	{fig:G:brick:LineFeed}%
	{1.3\textwidth}%
	{\textheight}

\clearpage



==> bricksInsideZagBlocks.tex <==
%!TEX root =  icalp2018.tex



{
\newcommand{\scaleBlock}{.5} %.2
\newcommand{\scaleBrick}{.5} %.5
\newcommand{\figBricks}[1]{\includegraphics[scale=\scaleBrick]{bricks/#1}}
\newcommand{\figBlocks}[1]{\includegraphics[scale=\scaleBlock]{blocks/#1}}
\newcommand{\figBlocksColor}[1]{\includegraphics[scale=\scaleBlock]{blocks-colored/#1}}
\newcommand{\figFontSize}{\small}
\newcommand{\flipFig}[3]{%
	\settoheight{\figHeight}{#3}
	\raisebox{\figHeight}{\scalebox{#1}[#2]{#3}}
}%
\newcommand{\NotApplicable}[1]{\raisebox{#1}{\textit{\figFontSize\sffamily N\!/\!A}}}
\newcommand{\figModule}[2]{\raisebox{#1}{\figFontSize #2}}
\newcommand{\figLegend}[1]{\scalebox{.8}{\figFontSize #1}}
\newcommand{\figBrickRef}[2]{\makebox[0em][r]{\scriptsize\sffamily(see Figure~\ref{#1})\hspace*{#2}}}
\newcommand{\nameit}[2]{\hspace*{#2}{\scriptsize #1}}
\newcommand{\figBrickReff}[3]{\makebox[0em][r]{\sffamily\begin{tabular}[b]{r}\nameit{#3}{0mm}\\[-1mm]\scriptsize (see Figure~\ref{#1})\end{tabular}\hspace*{#2}}}


%%%
%%% ZAG
%%%

\begin{tabular}{rrcccccc}
%\multicolumn{8}{c}{\bfseries Zag}
%\\
%
\toprule
%
\multicolumn{1}{c}{\bZag\,Zag-Block}
&	\multicolumn{1}{c}{\makebox[0em][r]{Modules:\quad} \ModuleG}
&	\ModuleF
&	\ModuleE
&	\ModuleDx{}
&	\ModuleC
&	\ModuleB
&	\ModuleA
\\[1mm] 
%
\toprule
%
\figBlocksColor{COPY0Zag-color.pdf}
&	\raisebox{-17mm}[0mm][0mm]{\flipFig{-1}{1}{\figBricks{G-ZIGCOPY0.pdf}} \flipFig{-1}{1}{\figBricks{G-ZIGCOPY1.pdf}}}
&	\flipFig{-1}{-1}{\figBricks{F-ZIGUP.pdf}}
&	\flipFig{-1}{-1}{\figBricks{E-ZIGUP.pdf}}
&	\raisebox{6mm}{\flipFig{-1}{-1}{\figBricks{D0-ZIGUP.pdf}} \flipFig{-1}{-1}{\figBricks{D1-ZIGUP.pdf}}}
&	\flipFig{-1}{-1}{\figBricks{C-ZIGUP.pdf}}
&	\flipFig{-1}{-1}{\figBricks{B-ZIGUP.pdf}}
&	\flipFig{-1}{-1}{\figBricks{A-ZIGUP.pdf}}
\\ 
\multicolumn{1}{c}{\bkZAGCOPY{\word0}} 
&	\multicolumn{1}{c}{$\GZagCopyZ$ $\GZagCopyU$}
&	$\FZag$
&	$\EaZag{\ensuremath{a}}$
&	$\DZZag{r,t}$ $\DUZag{r,t}$
&	$\CZag$
&	$\BZag$
&	$\AZag$
\\[2mm]
%
\midrule
%
\figBlocksColor{COPY1Zag-color.pdf}
&	\raisebox{-17mm}[0mm][0mm]{\flipFig{-1}{1}{\figBricks{G-ZIGCOPY1.pdf}}}
&	\flipFig{-1}{-1}{\figBricks{F-ZIGUP.pdf}}
&	\flipFig{-1}{-1}{\figBricks{E-ZIGUP.pdf}}
&	\raisebox{6mm}{\flipFig{-1}{-1}{\figBricks{D0-ZIGUP.pdf}} \flipFig{-1}{-1}{\figBricks{D1-ZIGUP.pdf}}}
&	\flipFig{-1}{-1}{\figBricks{C-ZIGUP.pdf}}
&	\flipFig{-1}{-1}{\figBricks{B-ZIGUP.pdf}}
&	\flipFig{-1}{-1}{\figBricks{A-ZIGUP.pdf}}
\\ 
\multicolumn{1}{c}{\bkZAGCOPY{\word1}}  
&	$\GZagCopyU$
&	$\FZag$
&	$\EaZag{\ensuremath{a}}$
&	$\DZZag{r,t}$ $\DUZag{r,t}$
&	$\CZag$
&	$\BZag$
&	$\AZag$
\\[2mm]
%
\midrule
%
\raisebox{-17mm}{\figBlocksColor{COPY0ZagLF-color.pdf}}
&	\raisebox{-17mm}[0mm]{\figBricks{G-LF.pdf} \flipFig{-1}{1}{\figBricks{G-ZIGCOPY0.pdf}} \flipFig{-1}{1}{\figBricks{G-ZIGCOPY1.pdf}}}
&	\flipFig{-1}{-1}{\figBricks{F-ZIGUP.pdf}}
&	\flipFig{-1}{-1}{\figBricks{E-ZIGUP.pdf}}
&	\raisebox{6mm}{\flipFig{-1}{-1}{\figBricks{D0-ZIGUP.pdf}} \flipFig{-1}{-1}{\figBricks{D1-ZIGUP.pdf}}}
&	\flipFig{-1}{-1}{\figBricks{C-ZIGUP.pdf}}
&	\flipFig{-1}{-1}{\figBricks{B-ZIGUP.pdf}}
&	\flipFig{-1}{-1}{\figBricks{A-ZIGUP.pdf}}
\\ 
\multicolumn{1}{c}{\bkZAGCOPYLF{\word0}}  
&	\multicolumn{1}{c}{$\GLF$ $\GZagCopyZ$ $\GZagCopyU$}
&	$\FZag$
&	$\EaZag{\ensuremath{a}}$
&	$\DZZag{r,t}$ $\DUZag{r,t}$
&	$\CZag$
&	$\BZag$
&	$\AZag$
\\[2mm] 
%
\midrule
%
\raisebox{-17mm}{\figBlocksColor{COPY1ZagLF-color.pdf}}
&	\raisebox{-17mm}[0mm]{\figBricks{G-LF.pdf} \flipFig{-1}{1}{\figBricks{G-ZIGCOPY1.pdf}}}
&	\flipFig{-1}{-1}{\figBricks{F-ZIGUP.pdf}}
&	\flipFig{-1}{-1}{\figBricks{E-ZIGUP.pdf}}
&	\raisebox{6mm}{\flipFig{-1}{-1}{\figBricks{D0-ZIGUP.pdf}} \flipFig{-1}{-1}{\figBricks{D1-ZIGUP.pdf}}}
&	\flipFig{-1}{-1}{\figBricks{C-ZIGUP.pdf}}
&	\flipFig{-1}{-1}{\figBricks{B-ZIGUP.pdf}}
&	\flipFig{-1}{-1}{\figBricks{A-ZIGUP.pdf}}
\\
\multicolumn{1}{c}{\bkZAGCOPYLF{\word1}}  
&	\multicolumn{1}{c}{$\GLF$ $\GZagCopyU$}
&	$\FZag$
&	$\EaZag{\ensuremath{a}}$
&	$\DZZag{r,t}$ $\DUZag{r,t}$
&	$\CZag$
&	$\BZag$
&	$\AZag$
\\[2mm]
%
\bottomrule
%
\end{tabular}


}




==> bricksInsideZigBlocks.tex <==
%!TEX root =  icalp2018.tex



{
\newcommand{\scaleBlock}{.5} %.2
\newcommand{\scaleBrick}{.5} %.5
\newcommand{\figBricks}[1]{\includegraphics[scale=\scaleBrick]{bricks/#1}}
\newcommand{\figBlocks}[1]{\includegraphics[scale=\scaleBlock]{blocks/#1}}
\newcommand{\figBlocksColor}[1]{\includegraphics[scale=\scaleBlock]{blocks-colored/#1}}
%
\newcommand{\newscaleBlock}{.07} %.2
\newcommand{\newscaleBrick}{.07} %.5
\newcommand{\myN}{4}
\newcommand{\myL}{3}
\newcommand{\myP}{1}
\newcommand{\nameBrickFile}[2]{Module-#1-#2_n=\myN-L=\myL-P=\myP-arrow.pdf}
\newcommand{\newfigBrick}[2]{\includegraphics[scale=\newscaleBrick]{\nameBrickFile{#1}{#2}}}
\newcommand{\figFontSize}{\small}
\newcommand{\flipFig}[3]{%
	\settoheight{\figHeight}{#3}
	\raisebox{\figHeight}{\scalebox{#1}[#2]{#3}}
}%
\newcommand{\NotApplicable}[1]{\raisebox{#1}{\textit{\figFontSize\sffamily N\!/\!A}}}
\newcommand{\figModule}[2]{\raisebox{#1}{\figFontSize #2}}
\newcommand{\figLegend}[1]{\scalebox{.8}{\figFontSize #1}}
\newcommand{\figBrickRef}[2]{\makebox[0em][r]{\scriptsize\sffamily(see Figure~\ref{#1})\hspace*{#2}}}
\newcommand{\nameit}[2]{\hspace*{#2}{\scriptsize #1}}
\newcommand{\figBrickReff}[3]{\makebox[0em][r]{\sffamily\begin{tabular}[b]{r}\nameit{#3}{0mm}\\[-1mm]\scriptsize (see Figure~\ref{#1})\end{tabular}\hspace*{#2}}}

%%%
%%% ZIG
%%%

\begin{tabular}{cccccccc}
%\multicolumn{8}{c}{\bfseries Zig}
%\\
%
\toprule
%
Zig\,\bZig-Block
&	\makebox[0em][r]{Modules:\quad} \ModuleA
&	\ModuleB
&	\ModuleC
&	\ModuleDx{}
&	\ModuleE
&	\ModuleF
&	\ModuleG
\\[1mm] 
%
\toprule
%
\figBlocksColor{READ0-color.pdf}
&	\newfigBrick{A}{ZigUp}
&	\raisebox{16.5mm}{\figBricks{B-ZIGUP.pdf}}
&	\figBricks{C-ZIGUP.pdf}
&	\figBricks{D0-ZIGUP.pdf} \figBricks{D1-ZIGUP.pdf}
&	\figBricks{E-ZIGUP.pdf}
&	\figBricks{F-ZIGUP.pdf}
&	\figBricks{G-READ0.pdf}
\\ 
\multicolumn{1}{c}{\bkREAD{\word0}} 
&	$\AZigUp$
&	$\BZigUp$
&	$\CZigUp$
&	$\DZZigUp{r,t}$ $\DUZigUp{r,t}$
&	$\EaZigUp{\ensuremath{a}}$
&	$\FZigUp$
&	$\GReadZ$
\\[2mm]
%
\midrule
%
\figBlocksColor{READ1-color.pdf}
&	\figBricks{A-ZIGUP.pdf}
&	\raisebox{16.5mm}{\figBricks{B-ZIGUP.pdf}}
&	\figBricks{C-ZIGUP.pdf}
&	\figBricks{D0-ZIGUP.pdf} \figBricks{D1-ZIGUP.pdf}
&	\figBricks{E-ZIGUP.pdf}
&	\figBricks{F-ZIGUP.pdf}
&	\figBricks{G-READ1.pdf}
\\ 
\multicolumn{1}{c}{\bkREAD{\word1}} 
&	$\AZigUp$
&	$\BZigUp$
&	$\CZigUp$
&	$\DZZigUp{r,t}$ $\DUZigUp{r,t}$
&	$\EaZigUp{\ensuremath{a}}$
&	$\FZigUp$
&	$\GReadU$
\\[2mm]
%
\midrule
%
\figBlocksColor{COPY0Zig-color.pdf}
&	\flipFig{1}{-1}{\figBricks{A-ZIGUP.pdf}}
&	\flipFig{1}{-1}{\figBricks{B-ZIGUP.pdf}}
&	\flipFig{1}{-1}{\figBricks{C-ZIGUP.pdf}}
&	\raisebox{6mm}{\flipFig{1}{-1}{\figBricks{D0-ZIGUP.pdf}} \flipFig{1}{-1}{\figBricks{D1-ZIGUP.pdf}}}
&	\flipFig{1}{-1}{\figBricks{E-ZIGUP.pdf}}
&	\flipFig{1}{-1}{\figBricks{F-ZIGUP.pdf}}
&	\figBricks{G-ZIGCOPY0.pdf} \figBricks{G-ZIGCOPY1.pdf}
\\ 
\multicolumn{1}{c}{\bkZIGCOPY{\word0}} 
&	$\AZigDown$
&	$\BZigDown$
&	$\CZigDown$
&	$\DZZigDown{r,t}$ $\DUZigDown{r,t}$
&	$\EaZigDown{\ensuremath{a}}$
&	$\FZigDown$
&	$\GZigCopyZ$ $\GZigCopyU$
\\[2mm]
%
\midrule
%
\figBlocksColor{COPY1Zig-color.pdf}
&	\flipFig{1}{-1}{\figBricks{A-ZIGUP.pdf}}
&	\flipFig{1}{-1}{\figBricks{B-ZIGUP.pdf}}
&	\flipFig{1}{-1}{\figBricks{C-ZIGUP.pdf}}
&	\raisebox{6mm}{\flipFig{1}{-1}{\figBricks{D0-ZIGUP.pdf}} \flipFig{1}{-1}{\figBricks{D1-ZIGUP.pdf}}}
&	\flipFig{1}{-1}{\figBricks{E-ZIGUP.pdf}}
&	\flipFig{1}{-1}{\figBricks{F-ZIGUP.pdf}}
&	\figBricks{G-ZIGCOPY1.pdf}
\\
\multicolumn{1}{c}{\bkZIGCOPY{\word1}} 
&	$\AZigDown$
&	$\BZigDown$
&	$\CZigDown$
&	$\DZZigDown{r,t}$ $\DUZigDown{r,t}$
&	$\EaZigDown{\ensuremath{a}}$
&	$\FZigDown$
&	$\GZigCopyU$
\\[2mm]
%
\midrule
%
\multicolumn{1}{r}{\figBlocksColor{APPEND01LF-color.pdf}}
&	\raisebox{16.5mm}{\flipFig{1}{-1}{\figBricks{A-ZIGUP.pdf}}}
&	\raisebox{16.5mm}{\flipFig{1}{-1}{\figBricks{B-ZIGUP.pdf}}}
&	\raisebox{16.5mm}{\figBricks{C-END.pdf}}
&	\raisebox{9mm}{\begin{tabular}[b]{c}
		\figBricks{D-WRITE0-0.pdf}\\
		\figBricks{D-WRITE1-0.pdf}\\
		\figBricks{D-WRITE0-1.pdf}\\
		\figBricks{D-WRITE1-1.pdf}
	\end{tabular}}
&	\raisebox{12,5mm}{\begin{tabular}[b]{c}
		\figBricks{E-CR-0.pdf}\\
		\figBricks{E-CR-1.pdf}
	\end{tabular}}
&	\flipFig{-1}{-1}{\figBricks{F-ZIGUP.pdf}}
&	\raisebox{-17.5mm}[10mm][0mm]{\flipFig{-1}{1}{\figBricks{G-ZIGCOPY1.pdf}}}
\\ 
\multicolumn{1}{c}{\bkAPPENDRETURN{(\alpha)}} 
&	$\AZigDown$
&	$\BZigDown$
&	$\CEnd$
&	$\DZAppend{r,t}$ $\DUAppend{r,t}$
&	$\EaCR{\ensuremath{a}}$
&	$\FZag$
&	$\GZagCopyU$
\\[2mm]
%
\midrule
%
\figBlocksColor{HALT-color.pdf}
&	\figBricks{A-ZIGUP.pdf}
&	\raisebox{16.5mm}{\figBricks{B-EMPTY.pdf}}
\\ 
\bkHALT
&	$\AZigUp$
&	$\BHalt$
\\[2mm]
%
\midrule
%
\figBlocksColor{AppendeCRLF_n=4_l=2_p=0_w=30_h=111.pdf}
&	\raisebox{37mm}{\flipFig{1}{-1}{\figBricks{A-ZIGUP.pdf}}} \figBricks{A-ZIGUP.pdf}
&	\raisebox{16.5mm}{\begin{tabular}[b]{c}\flipFig{1}{-1}{\figBricks{B-ZIGUP.pdf}}\\[16mm] \figBricks{B-EMPTY.pdf}\end{tabular}}
&	\raisebox{37mm}{\figBricks{C-END.pdf}}
&	\raisebox{30mm}{\begin{tabular}[b]{c}
		\figBricks{D-WRITE0-0.pdf}\\
		\figBricks{D-WRITE1-0.pdf}\\
		\figBricks{D-WRITE0-1.pdf}\\
		\figBricks{D-WRITE1-1.pdf}
	\end{tabular}}
&	\raisebox{30mm}{\begin{tabular}[b]{c}
		\figBricks{E-CR-0.pdf}\\
		\figBricks{E-CR-1.pdf}
	\end{tabular}}
&	\raisebox{16.5mm}{\flipFig{-1}{-1}{\figBricks{F-ZIGUP.pdf}}}
&	\raisebox{0mm}{\figBricks{G-LF.pdf}}
\\
\bkRETURNLINEFEEDHALT 
&	$\AZigDown$ $\AZigUp$
&	$\BZigDown$ $\BHalt$
&	$\CEnd$
&	$\DZAppend{r,t}$ $\DUAppend{r,t}$
&	$\EaCR{\ensuremath{a}}$
&	$\FZag$
&	$\GZagCopyU$
\\[2mm]
%
\bottomrule
%
\end{tabular}
}




==> modules.tex <==
%!TEX root =  icalp2018.tex

%%% --------------------------------------------------------------------------------
\section{Full description of the SCTS oritatami simulator}
%%% --------------------------------------------------------------------------------

Consider a SCTS $\TMS$ with $n$ appendants $\alpha_0, \ldots, \alpha_{n-1}\in\{\word0, \word1\}^*$ , where $n$ is at least $8$ and a multiple of~$4$, together with an input dataword $u\in\{\word0, \word1\}^*$.

We give here the full description of the primary structure $\pi_\TMS$ of the oritatami systems $\TMO_\TMS=((\pi_\TMS)^\infty, \heart, 3)$ together with its seed conformation $\sigma_\TMS(u)$, which simulates step by step the computation of~$\TMS$ on input dataword~$u$.
 
\subparagraph{Convenience variables.} 
In order to simplify the description, we introduce the following variables which correspond to key geometrical parameters of the different modules:  %Recall that $n$ is the number of appendants in $\TMS$ and that $n$ is assumed to be at least $8$ and a multiple of $4$. 

\begin{align*}
L	
&	= \max_{0\leq i< n} |\alpha_i|
&	\text{the maximum length of an appendant in $\TMS$}
\\
P
&	 = 12-(L\mod 2)
&	\text{ the \emph{padding} constant, such that $L+P$ is even and at least $12$}
\\
w
&	= 6(L+P)+18
&	\text{the width of the appendant module excluding its read/copy/linefeed part}
\\
W
&	= n\cdot (w+6)
&	\text{the width of the \bnREAD{}{}, \bnZIGCOPY{}{}, and \bnZAGCOPY{}{} blocks}
\\
h
&	= W-(w+3)
&	\text{the height of the zig and zag rows}
\\
k
&	= (h-3)/6
&	\text{the number of periods of a glider of length $h$}
\\
\lambda
&	= W/2
&	\text{\makebox[0em][r]{the} height of the letter modules inside the \bnREAD{}{}, \bnZIGCOPY{}{}, and \bnZAGCOPY{}{} blocks}
\\
\kappa
&	= W/24
&	\begin{array}[t]{r@{}}
		\text{the number of periods of the glider/switchback pattern}\\
		\text{in the letter and padding modules}
	\end{array}
\\
q
&	= (h-3)/4
&	\text{the number of periods of the glider in the backbone of module $\ModuleE$}
\\
c(a)
&	= \makebox[0em][l]{$(6\lambda(L-a+P)+8h-16)/4$}
&	\text{the width of the brick $\EaCR{a}$ }
\end{align*}

As $n$ is a multiple of $4$ and as $L+P$ is even, we have: 
\begin{fact}
All convenience variables $L, P, w, W, h, k, \lambda, \kappa, q, c(a)$ are integers. Furthermore, 
%
$$
\begin{array}{r@{~}c@{~}lr@{~}c@{~}lr@{~}c@{~}lr@{~}c@{~}l}
	w& =& 6 \mod 12,
&	W& = &0 \mod 48,
&	 h &= &3 \mod 12,
&	k &=& 0\mod 2,
\\
	\lambda &= &0 \mod 24,
&	\kappa &=& 0 \mod 2,
&	q &=& 0 \mod 3,
&	c(a)& =& 2 \mod 12 \text{, for all $0\leq a\leq L$.}
\end{array}
$$
\end{fact}


\subparagraph{Notations for describing of the bead type sequences.}
if $u$ and $v$ are two finite bead type sequences, we write their concatenation as $u\cdot v$. For any two integers $0\leq i\leq j<|u|$, we write $u_{i\ldots j}$ for $u_iu_{i+1}\ldots u_j$. The \emph{reverse sequence} of $u$, written as $u^R$, is $u_{|u|-1}u_{|u|-2}\ldots u_1 u_0$.

  Finally, given a sequence $u$, we write $u\subst{a_1\!@i_1,\ldots, a_k\!@i_k}$ for the sequence $w$ where  the bead type indexed by $i_j$ in $u$ has been replaced by $a_j$ for $j=1,\ldots,k$:
$$
w_i = \left\{
  \begin{array}{cl}
    a_j	&\text{if $i = i_j$ for some $j$}\\
    u_i	&\text{otherwise} 
  \end{array}
\right.
$$

By extension, we write $u\subst{v@{k..l}}$ for the sequence $w$ where for all $i\in\{k,k+1, \ldots, l\}$, the beads at indices $k$ to $l$ of $u$ have been replaced by the word $v$ (of length $l-k+1$):
$$
w_i = \left\{
  \begin{array}{cl}
    v_{i-k}	&\text{if $k\leq i \leq l$}\\
    u_i	&\text{otherwise} 
  \end{array}
\right.
$$

For an infinite sequence of (finite) words $(u_i)_{i\geq1}$, we denote by $\concatop_{i\geq1}u_i$ the infinite word $u_1 u_2\cdots u_i\cdots$ obtained by containing all the words $u_1,u_2,\ldots$


%%%%%%% --------------------------------------------------------------------------------
\subsection{The periodic primary structure  $(\pi_\TMS)^\infty$}
%%%%%%% --------------------------------------------------------------------------------

The period of the primary structure consists in the concatenation of one appendant bead type sequence for each appendant:
%
$$ 
\pi_\TMS 
= \APPENDANTa{0}\conc\APPENDANTa{1}\conc \,\cdots \, \conc \APPENDANTa{n-1}
$$


%%%%%%% --------------------------------------------------------------------------------
\subsection{The appendant bead type sequences}
%%%%%%% --------------------------------------------------------------------------------

Each appendant bead type sequence $\APPENDANTa{i}$ has the exact same structure: it is the concatenation of 6 sequences: Modules \ModuleA, \ModuleB, and \ModuleC, followed a sequence \WORD{\alpha_i} encoding the appendant~$\alpha_i$ itself, followed by modules  \ModuleF\/ and \ModuleG:
%
$$
\APPENDANTa{i}
=	\ModuleA \conc \ModuleB \conc \ModuleC \conc \WORD{\alpha_i} \conc \ModuleF \conc \ModuleG
$$
%
For each word $v\in\{\word0,\word1\}^*$ with $|v|\leq L$, \WORD{v} encodes each letter of $v$ using one of the 6 variants of module \ModuleDx{} and terminates with a padding sequence \ModuleEa{L-|v|} which ensures that the folded size of $\WORD{v}$ is independent of the length of~$v$. The 6 variants of the module \ModuleDx{} are \ModuleDx{x,r,t} where:
%
\begin{itemize}[topsep=2pt,itemsep=0pt]
%
\item $x\in\{\word0,\word1\}$  is the encoded letter; 
%
\item $r\in\{0,1,2\}$ is the rank of the letter inside the encoded word $v$: $r=0$ if it is the first letter of $v$; $r=1$ if its index in $v$ is odd; and $r=2$ if its index in $v$ is even but not $0$;
%
\item $t\in\{0,1\}$ is $1$ if the encoded letter is the last letter of $v$, and $0$ otherwise.
\end{itemize}
%
The definition of the sequence \WORD{v} follows as: 
%
\begin{align*}
\WORD\epsilon
&	= \ModuleEa{L}
\\
\WORD{\word0}
&	= \ModuleDZ{0,1} \conc \ModuleEa{L-1}
\\
\WORD{\word1}
&	= \ModuleDU{0,1} \conc \ModuleEa{L-1}
\\
\text{and for $|v|\geq 2$,\quad}
\WORD{v}
&	= \ModuleDx{v_0,0,0} 
	\conc \left( \concatup{i=1}{|v|-2} \ModuleDx{v_i, 2-(i\,\mod\,2), 0}\right) 
	\conc \ModuleDx{v_{n-1}, 2-((|v|-1)\,\mod\,2), 1} 
	\conc \ModuleEa{L-|v|}
\end{align*}

The next section concludes the full description of the primary structure by giving the sequences for modules \ModuleA, \ModuleB, \ModuleC, \ModuleDx{x,r,t}, \ModuleEa{a}, \ModuleF, and \ModuleG.    

%%%%%%% --------------------------------------------------------------------------------
\subsection{Modules bead type sequences}
%%%%%%% --------------------------------------------------------------------------------

The modules are given using $546$ bead types. However, 5 of them, \bA6, \bC{16}, \bJ{9}, \bL{86}, and \bL{89}, are \emph{neutral}, i.e. do not have any interaction with any other bead types (see Section~\ref{sec:rule}) and can thus be all substituted by one single \emph{neutral} bead type $\bN0$. The total number of distinct bead types is thus $542$ ($541$ + $1$ neutral bead type $\bN0$).  However, in the description bellow, we prefer to use \bA6, \bC{16}, \bJ{9}, \bL{86}, and \bL{89} (and not $\bN0$) as it keeps the bead types homogenous  and continuously numbered in each module. 

%\paragraph{Module $\protect\ModuleA$:} 
\subsubsection{Module A} 
Length: $3h-2$; 13 bead types used: $\bbA{0}{12}$
$$
\ModuleA =  \bSN{\bbA{0}{4}}\conc (\bbA{5}{10})^{3k-1}\conc \bbA{5}{7} \conc \bSN{\bA{6}}\conc \bbA{9}{10} \conc \bSN{\bbA{11}{12}}
$$
	
%\paragraph{Module $\protect\ModuleB$:} 
\subsubsection{Module B} 
Length: $5$; 5 bead types used: $\bbB{0}{4}$
$$
\ModuleB =  \bbB{0}{4}
$$
	
%\paragraph{Module $\protect\ModuleC$:} 
\subsubsection{Module C} 
Length: $3h-10$; 17 bead types used: $\bbC{0}{16}$
$$
 \ModuleC = (\bbC{0}{2})^{2k}\conc (\bbC{3}{5})^{k}\conc \bC3\conc \bbC{7}{8}\conc (\bbC{6}{8})^{k-1}\conc (\bbC{9}{14})^{k-1}\conc \bbC{9}{10}\conc \bSN{\bbC{15}{16}} \conc \bC{13}
 $$

%\paragraph{Modules $\protect\ModuleDx{x,r,t}$:} 
\subsubsection{Modules D} 
Length: $3W+30 = 6(\lambda+5)$;\\ uses: 111 proper bead types, $\bbD{0}{62}$ and $\bbE{0}{47}$; plus 2 special bead types from~\ModuleG, $\bbL{17}{18}$

\begin{align*}
\SEGD0 & =  \bSB{\bbD{23}{33}}\conc \bbE{6}{11}\conc (\bbE{0}{11})^{\kappa-1}
\\
\SEGD1 & =  (\bbE{12}{23})^{\kappa}\conc \bSB{\bbD{49}{45}}
\\
\SEGD2 & =  \bSB{\bbD{34}{44}}\conc \bbE{30}{35}\conc (\bbE{24}{35})^{\kappa-1}
\\
\SEGD3 & =  (\bbE{36}{47})^{\kappa}\conc \bSB{\bbD{54}{50}}
\\
\ModuleDU{2,0} 
&	= \SEGD0\conc \SEGD1\conc  \SEGD2\conc \SEGD3\conc  \SEGD0\conc \SEGD1
\\
\ModuleDU{1,0} 
&	= \SEGD2\conc \SEGD3\conc  \SEGD0\conc \SEGD1\conc \SEGD2\conc \SEGD3
\\ 
\ModuleDU{0,0} 
&	= \ModuleDU{2,0}\subst{\bS{\bbD{0}{16}}@0..16}
\\
\ModuleDU{r,1} 
&	= \ModuleDU{r,0}\subst{\bS{\bD{17}}@(3W+22), \bS{\bbD{18}{22}}@(3W+25)..(3W+29)} 
& 	\text{for $r\in\{0,1,2\}$}
\\
\ModuleDZ{r,t} 
&	= \ModuleDU{r,t}\subst{\bS{\bL{17}}@(3w+1), \bS{\bL{18}}@(3w+2), \bSP{\bbD{55}{62}}@(3w+6)..(3w+13)}
& 	\begin{array}[t]{r} 
		\text{for $r\in\{0,1,2\}$}
		\\
		\text{and $t\in\{0,1\}$}
	\end{array}
\end{align*}
	
%\paragraph{Modules \protect\ModuleEa{a}:} 
\subsubsection{Modules E} 
Length: $6\lambda(L-a+P)+8h-1$; \\ 
146 bead types used: $\bbF{0}{51}$, $\bbG{0}{48}$, $\bbH{0}{24}$, and $\bbI{0}{19}$.
%
\begin{align*}
\SEGE{A} 
&	= \bigl((\bbF{0}{11})^\kappa \conc (\bbF{12}{23})^\kappa \conc (\bbF{24}{35})^\kappa \conc (\bbF{36}{47})^\kappa\bigr)^\infty
\\
\SEGE{B} 
&	= \bigl((\bbG{0}{11})^\kappa \conc (\bbG{12}{23})^\kappa \conc (\bbG{24}{35})^\kappa \conc (\bbG{36}{47})^\kappa\bigr)^\infty
\\
\HEAD{E$_a$} 
&	= \SEGE{A}_{b..b+3c(a)-2} \conc \bS{\bF{51}} \conc \SEGE{B}_{b+3c(a)..b+K-2}
&	\begin{array}[t]{r} 
		\text{\quad where $b= 0$ if $a$ is even,}
		\\ 
		\text{and $b=2\lambda$ if $a$ is odd}
		\end{array}
\\[2mm]
\SEGE{C} 
&	= \bSN{\bbH{0}{4}} \conc (\bbH{5}{16})^{q-1} \conc \bbH{5}{10} \conc \bSC{\bbH{17}{24}}
\\
\SEGE{D$_0$}
&	= \bSC{\bI{15}} \conc \bbI{1}{5} \conc (\bbI{0}{5})^{k-1} \conc \bbI{0}{1} \conc \bSC{\bI{18}}
\\
\SEGE{D$_1$} 
&	= \bSC{\bI{19}} \conc \bbI{7}{8} \conc (\bbI{6}{8})^{2k-1}\conc \bbI{6}{7}\conc \bSC{\bbI{15}{16}}
\\
\SEGE{D$_2$}
&	= \bSC{\bI{17}}\conc \bbI{10}{11} \conc (\bbI{9}{11})^{2k-1} \conc \bbI{9}{10}\conc \bSC{\bI{19}}
\\
\SEGE{D$_3$}
&	= \bSC{\bI{18}} \conc \bbI{13}{14} \conc (\bbI{12}{14})^{2k-1} \conc \bbI{12}{13} \conc \bSC{\bI{19}}
\\
\SEGE{D$_4$}
&	= \bSC{\bI{19}} \conc \bbI{1}{2} \conc (\bbI{0}{2})^{2k}
\\
\TAIL{E} 
&	= \SEGE{C} \conc \SEGE{D$_0$} \conc \SEGE{D$_1$} \conc \SEGE{D$_2$} \conc \SEGE{D$_3$} \conc \SEGE{D$_4$}
\\[2mm]
\ModuleEa{0} 
&	= \HEAD{E$_0$}\subst{\bS{\bbF{48}{49}}@0..1, \bS{\bF{50}}@11} \conc \bS{\bG{48}} \conc \TAIL{E}
\\
\ModuleEa{a>0} 
&	= \HEAD{E$_{a}$}\conc \bS{\bG{48}} \conc \TAIL{E}
\end{align*}

%\paragraph{Module \protect\ModuleF:} 
\subsubsection{Module F} 
Length: $4h$; 53 bead types used: $\bbJ{0}{52}$.
%
\begin{align*}
\HEAD F 
&	= \bSN{\bbJ{0}{4}} \conc (\bbJ{5}{10})^{3k-1} \conc \bbJ{5}{7} \conc \bSN{\bbJ{11}{23}}
\\
\TAIL F 
&	= \bJ{48} \conc (\bbJ{51}{48})^{9} \conc \bJ{51} \conc \bSN{\bJ{52}} \conc \bbJ{49}{48}
\\[2mm]
\SEG{Exp}{$(2i)$} 
&	= \bSE{\bbJ{24}{29}} \conc (\bbJ{30}{35})^{3^{2i-1}-1}
&	\text{for $i\geq 1$}
\\
\SEG{Exp$(2i+1)$}{} 
&	= \bSE{\bbJ{36}{41}} \conc (\bbJ{42}{47})^{3^{2i}-1}
&	\text{for $i\geq 1$}
\\
\SEG{Exp}{F} 
&	= \concat{i\geq2}  \SEG{Exp$(i)$}{}
\\%[2mm]
\ModuleF 
&	= \HEAD F \cdot \left(\bSE{\bbJ{39}{41}}\conc \SEG{Exp}{F}_{0..(h-51)}\right)^R \conc  \TAIL F
\end{align*}

%\paragraph{Module \protect\ModuleG:} 
\subsubsection{Module G} 
Length: $6h-1$;  201 bead types used: $\bbK{0}{69}$, $\bbL{0}{99}$, and $\bbM{0}{30}$.

\begin{align*}
\SEG{Exp'}{$(2i)$} 
&	= \bSE{\bbK{4}{9}} \conc (\bbK{10}{15})^{3^{2i-1}-1}
&	\text{for $i\geq 1$}
\\
\SEG{Exp'}{$(2i+1)$} 
&	= \bSE{\bbK{16}{21}} \conc (\bbK{22}{27})^{3^{2i}-1}
&	\text{for $i\geq 1$}
\\
\SEG{Exp}{G} 
&	= \concat{i\geq2}  \SEG{Exp'}{$(i)$}  
\\[1mm]
\SEG G1 
&	= \bS{\bbL{0}{6}} \conc \bK3 \conc (\bbK{0}{3})^9 \conc \bbK{0}{2} \conc \bS{\bbL{7}{10}} \conc \SEG{Exp}{G}_{8..h-51}
\\
\SEG G2 
&	= \bK{32} \conc \bK{33}\conc (\bbK{28}{33})^{k-3} \conc \bbK{28}{32}
\\
\SEG G3 
&	= \begin{array}[t]{l} 
		\bbK{35}{39} \conc (\bbK{34}{39})^{k-14}\conc \bK{34}\conc \bK{35} \conc \bSR{\bbL{39}{41}} \conc \bK{45} \conc (\bbK{40}{45})^{10}\, \conc
		\\ \quad
		  \bK{40}\conc \bK{41}
		  \end{array}
\\
\SEG G4
&	= \bbK{50}{51} \conc  (\bbK{46}{51})^{k-3}\conc \bbK{46}{48}
\\
\SEG G5
&	=  \begin{array}[t]{l} 
		\bbK{55}{57} \conc (\bbK{52}{57})^{k-6} \conc \bbK{52}{53} \conc \bS{\bL{74}\conc \bL{75}}  \conc \bbK{56}{57} \,\conc
		\\ \quad
		(\bbK{52}{57})^2 \conc \bbK{52}{53}
		\end{array}
\\
\SEG G6 
&	= \begin{array}[t]{l} 
		\bK{63}\conc (\bbK{58}{63})^{k-19} \conc \bbK{58}{61} \conc \bSC{\bbL{91}{99}\conc\bbM{0}{19}} \conc \bbK{67}{69} \, \conc 
		\\ \quad
		(\bbK{64}{69})^{10} \conc \bS{\bbM{20}{30}}
		\end{array}
\\[2mm]
\ModuleG 
&	= \SEG G1 \conc  \bS{\bbL{11}{24}}  \conc \SEG G{2}\conc  \bSCW{\bbL{25}{38}} \conc \SEG G{3}\conc  \bSCW{\bbL{42}{55}} \conc \SEG G{4}\, \conc\\
&	\hspace*{1cm}  \bSC{\bbL{56}{73}} \conc \SEG G{5} \conc  \bSC{\bbL{76}{90}} \conc \SEG G{6}
\end{align*}

%%%
%%%
%%%

\subparagraph{The seed conformation}	is described in the next section. 


